Advancing the State-of-the-Art in Hardware Trojans Design

Electronic Design Automation (EDA) industry heavily reuses third party IP cores. These IP cores are vulnerable to insertion of Hardware Trojans (HTs) at design time by third party IP core providers or by malicious insiders in the design team. State of the art research has shown that existing HT detection techniques, which claim to detect all publicly available HT benchmarks, can still be defeated by carefully designing new sophisticated HTs. The reason being that these techniques consider the HT landscape to be limited only to the publicly known HT benchmarks, or other similar (simple) HTs. However the adversary is not limited to these HTs and may devise new HT design principles to bypass these countermeasures. In this paper, we discover certain crucial properties of HTs which lead to the definition of an exponentially large class of Deterministic Hardware Trojans $H_D$ that an adversary can (but is not limited to) design. The discovered properties serve as HT design principles, based on which we design a new HT called 'XOR-LFSR' and present it as a 'proof-of-concept' example from the class $H_D$. These design principles help us understand the tremendous ways an adversary has to design a HT, and show that the existing publicly known HT benchmarks are just the tip of the iceberg on this huge landscape. This work, therefore, stresses that instead of guaranteeing a certain (low) false negative rate for a small constant set of publicly known HTs, a rigorous HT detection tool should take into account these newly discovered HT design principles and hence guarantee the detection of an exponentially large class (exponential in number of wires in IP core) of HTs with negligible false negative rate.

==> arxiv eprint/sections/abstract.tex <==
Electronic Design Automation (EDA) industry heavily reuses third party IP cores.
These IP cores are vulnerable to insertion of Hardware Trojans (HTs) at design time by third party IP core providers or by malicious insiders in the design team.
%These Trojans must be detected in pre-silicon phase, otherwise an adversary can infect millions of ICs through a Trojan affected IP core.
State of the art research has shown that existing HT detection techniques, which claim to detect all publicly available HT benchmarks, can still be defeated by carefully designing new sophisticated HTs.
The reason being that these techniques consider the HT landscape to be limited only to the publicly known HT benchmarks, or other similar (simple) HTs.
However the adversary is not limited to these HTs and may devise new HT design principles to bypass these countermeasures.

In this paper, we discover certain crucial properties of HTs which lead to the definition of an exponentially large class of Deterministic Hardware Trojans $H_D$ that an adversary can (but is not limited to) design.
The discovered properties serve as HT design principles, based on which we design a new HT called \textit{XOR-LFSR} and present it as a `proof-of-concept' example from the class $H_D$.
These design principles help us understand the tremendous ways an adversary has to design a HT, and show that the existing publicly known HT benchmarks are just the tip of the iceberg on this huge landscape.
This work, therefore, stresses that instead of guaranteeing a certain (low) false negative rate for a small \textit{constant} set of publicly known HTs, a rigorous HT detection tool should take into account these newly discovered HT design principles and hence guarantee the detection of an \textit{exponentially large} class (exponential in number of wires in IP core) of HTs with negligible false negative rate.



%We argue that those HTs that fall outside the characterized class $H_D$ use HT design principles that allow HTs which can never be detected within the pre-silicon logic testing based paradigm.

%Researchers have proposed some techniques to detect potentially a smaller subclass of this huge class, however these techniques are known to be computationally infeasible.
%This state of affairs leads to two crucial observations.
%First, instead of guaranteeing a certain (low) false negative rate for a small \textit{constant} set of publicly available benchmarks, a rigorous security framework of HTs should characterize which \textit{exponentially large} class (exponential in number of wires in IP core) of HTs a tool can detect with negligible false negative rate.
%Second, an effective detection tool must be designed which is computationally feasible for this class of HTs which is orders of magnitude larger compared to the small subclass (e.g. TrustHub) considered in the current literature.
%We present HaTCh, the first rigorous framework of HT design and detection within the paradigm of pre-silicon logic testing based tools.
%We first introduce certain crucial properties of HTs which lead to the characterization of an exponentially large class of HTs that an adversary can (but is not limited to) design, for which 
%We then develop and rigorously analyze HaTCh detection algorithm that detects any HT from $H_D$ class.
%Given certain global characteristics regarding the stealthiness of the HT within this class, the computational complexity of our algorithm for practical HTs scales polynomially with the number of wires in the IP core. %, as opposed to the exponential (in number of IP core inputs) complexity of current state of the art detection schemes to detect such HTs.
%We have implemented this algorithm, compared it with existing countermeasures, and tested it on TrustHub HT benchmarks, previously proposed HTs which alleviate state of the art detection schemes, and also on a newly designed advanced HT.




%We first characterize hardware trojans into two main groups called Deterministic and Non-Deterministic trojans and show that for non-deterministic hardware trojans, no (logic testing based) tool exists that, given a security parameter $\lambda$, can detect all trojans in this group with overwhelming probability $1-negl(\lambda)$.
%Then we propose, for the other (exponentially large) group of deterministic trojans/IP cores, a detection algorithm which detects \textit{any} hardware trojan from that group with overwhelming probability $1-negl(\lambda)$. If certain global characteristics regarding the stealthiness of such a hardware trojan are known, then detection becomes polynomial in the number of wires of the IP core.
%We implemented this algorithm and tested it on existing trojan benchmarks and also on a newly designed advanced trojan.


==> arxiv eprint/sections/background.tex <==

\section{Background \& Definitions}\label{sec:background-org}

\begin{figure}[!t]
\centering
\includegraphics[width=2.6in]{classification_a}
%\vspace{-6pt}
\caption{IP Core Design Space: An IP core can either have a Hardware Trojan or an Exploit, or it behaves `normally'.}
\label{fig:classification_a}
%\vspace{-12pt}
\end{figure}

%\subsection{IP Core Design Space} \label{sec:ip_design_space}
A digital IP core can fall under one of the following three categories, as shown in \figurename~\ref{fig:classification_a}, based on its level of conformity to the design specifications; (1) containing \textit{A Hardware Trojan}, or (2) containing \textit{An Exploit}, or (3) exhibiting \textit{Normal Behavior}. 

\subsection{Hardware Trojan}
A Hardware Trojan (HT) is malicious \textit{extra} circuitry embedded inside a larger circuit, which results in data leakage or harm to the normal functionality of the circuit once activated.
We define \textit{extra} circuitry as redundant logic added to the IP core without which the core can still meet its design specifications\footnote{Design specifications can also cover the performance requirements of the core, and hence pipeline registers etc. added to the core only for performance reasons can also be considered as `necessary' to meet the design specifications and will not be counted towards `extra' circuitry.}.
A \textit{trigger activated} HT activates upon some special event, whereas an \textit{always active} HT remains active all the time to deliver the intended payload.
%Once activated, a trojan can deliver its payload either through standard I/O channels or through side channels.

Trigger activated HTs typically consist of two parts: a \textit{trigger circuitry} and a \textit{payload circuitry}.
The trigger circuitry is implemented semantically as a comparator which compares the value(s) of certain wires(s) of the circuit with a specified boolean value called \textit{trigger condition}.
The HT trigger circuitry sends its comparator's output to the payload circuitry over certain other wire(s) called the \textit{trigger signal}.
Once the trigger signal is asserted, the payload circuitry performs the malicious operation called `payload' as intended by the adversary.

\begin{definition}
\textbf{Trigger condition} refers to an event, manifested in the form of a particular boolean value of certain internal/external wires of the circuit, which activates the HT trigger circuitry.
\end{definition}
\begin{definition}
\textbf{Trigger signal or Trigger State} refers to a collection of physical wire(s) which the HT trigger circuitry asserts in order to activate the payload circuitry once a trigger condition occurs.
\end{definition}

The trigger signal must not be confused with trigger condition; trigger condition is an event which causes the HT activation, whereas trigger signal is the output of trigger circuitry which tells the payload circuitry to show malicious behavior.

\begin{figure}[!t]
\centering
\subfloat[Half Adder]{\includegraphics[width=1.4in]{simple_ht_exp_1}
\label{fig:simple_ht_exp_1}}
\hfil
\subfloat[Half Adder with HT]{\includegraphics[width=1.9in]{simple_ht_exp_2}
\label{fig:simple_ht_exp_2}}
\caption{A simple HT: Trigger condition $A=B$; Normal output $S=A \oplus B$; Malicious output (under trigger condition) $S=B$.}
\label{fig:simple_ht_example}
\end{figure}

\figurename~\ref{fig:simple_ht_example} shows an example of a simple HT embedded in a half adder circuit.
The HT-free circuit in \figurename~\ref{fig:simple_ht_exp_1} generates a sum $S=A \oplus B$ and a carry $C=A \cdot B$. 
The HT, highlighted in red in \figurename~\ref{fig:simple_ht_exp_2}, triggers when $A=B$ and produces incorrect results i.e. $S=B$ for $A=B$ and $S=A \oplus B$ for $A \ne B$.
Notice the difference between the trigger condition $A=B$, and the trigger signal $Sel$ which only becomes $1$ when the trigger condition is satisfied.

The Trojan affected circuit in \figurename~\ref{fig:simple_ht_example} produces a \textit{malicious} output $S=1$ for trigger condition $A=B=1$ which is distinguishable from otherwise normal output ($S=0$). 
However, the same circuit produces a (so called) malicious output $S=0$ for trigger condition $A=B=0$ which is the same as otherwise normal output and cannot be distinguished from the `normal' behavior of the circuit.
This observation leads us to the definition of \textit{explicit} vs. \textit{implicit} malicious behaviors:

\begin{definition}
\textbf{Explicit malicious behavior} refers to a behavior of a HT where the HT generated output is \textit{distinguishable} from a normal output.
\end{definition}
\begin{definition}
\textbf{Implicit malicious behavior} refers to a behavior of a HT where the HT generated output is \textit{indistinguishable} from a normal output. 
\end{definition}

Notice that an adversary may exploit the implicit malicious behavior to bypass functional testing based detection tools during the testing phase.
Once the infected circuit has passed the testing and is deployed, it can then manifest explicit malicious behavior to actually deliver the payload.
In other words, implicit malicious behavior can lead to a false negative.

\begin{definition}
\textbf{False Negative} refers to a scenario when a HT detection tool identifies a circuit containing a HT as a Trojan-free circuit or transforms a circuit containing a HT into a circuit which still allows the HT to express implicit or explicit malicious behavior.
\end{definition}

Clearly, all existing dynamic analysis (i.e. functional testing) based approaches which assume that a HT is never triggered during the functional testing phase can suffer from false negatives because of the implicit malicious behavior.
Neglecting the implicit malicious behavior could lead to devastating consequences in a security critical application, e.g. if an adversary designs a HT to significantly increase the probability of implicit malicious behavior and thus alleviates the existing HT detection techniques.

\subsection{An Exploit}
An exploit refers to a loophole in the specifications or implementation of an IP core which allows an adversary to manipulate it beyond its intended specifications.
Notice that an exploitable IP core does not have `extra' circuitry like a Hardware Trojan.
Depending upon the nature of the exploits, they can also deliver the payloads like Hardware Trojans such as privacy leakage or denial of service etc.
Some examples of exploits are as follows: a wireless connection that can be overloaded may lead to a denial of service, a broken AES module due to a predictable key, recent OpenSSL Heartbleed bug etc. 
This paper only focuses on rigorous reasoning about Hardware Trojans (not exploits).

%\subsection{Threat Model}
%A third party IP core is provided in the form of a synthesized netlist which obfuscates the HDL source code.
%The IP core vendor has embedded a trigger based hardware trojan in the IP core which delivers its payload via standard IO channels of the IP core.
%The hardware trojan could have been inserted directly by maliciously modifying the source code or by using some malicious tools to synthesize the RTL.
%This IP core is used in a larger design whose millions of chips are fabricated.
%The adversary wants to exploit this scalability to infect millions of fabricated chips by supplying an infected IP core.
%To prevent this, we test the IP core for potential HTs in \textit{pre-silicon} phase, i.e. before integrating it into a larger design and fabricating it.
%Logic or functional testing, used by Design for Test (DFT) community for testing basic manufacturing defects, is one of the simplest methods to test the IP core for basic HTs which can be easily implemented using the existing simulation/testing tools.
%For the above reasons we restrict ourselves to analyzing logic testing based tools used in pre-silicon phase for HT detection.







==> arxiv eprint/sections/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
We provide the first rigorous framework of Hardware Trojans within which ``Deterministic Trojans'', the class $H_D$ is introduced.
We discover several stealthiness parameters of the Hardware Trojans from $H_D$ which lead us to design a much more stealthy \textit{XOR-LFSR} Hardware Trojan.
This shows that the current publicly known Hardware Trojans are the simplest ones in terms of stealthiness, and hence they represent just the tip of the iceberg at the huge landscape of Hardware Trojans.

We conclude that our framework allows the Hardware Trojan research community to rigorously reason about the stealthiness of different Hardware Trojans and the effectiveness of existing countermeasures.
The Hardware Trojan design principles introduced in this paper encourage and assist in designing new and even stronger countermeasures for highly stealthy and sophisticated Hardware Trojans.

==> arxiv eprint/sections/evaluation.tex <==
\section{Characterizing TrustHub Benchmarks}\label{sec:evaluation}

Trusthub~\cite{trust_hub} benchmark suite includes a wide variety of Hardware Trojans including trigger-activated and always-active Trojans; Trojans that use standard IO channels as well as side channels.
In this section, we analyze the TrustHub benchmarks with respect to our definitional framework.
As mentioned earlier, our $H_D$ class of HTs covers majority of the relevant benchmarks from TrushHub. 
Here we present the values of design parameters ($d$, $t$, $\alpha$) for these benchmarks which provide a deeper insight about the stealthiness of these well known HTs.



\begin{table}[t]
\renewcommand{\arraystretch}{1.2}
\setlength\tabcolsep{2pt}
\centering
\caption{Classification of Trusthub Benchmarks w.r.t. our definitional framework}
\label{table:trusthub_table}
\begin{tabular}{|c|c|c|c|c||m{0.7\columnwidth}|}\hline

\multicolumn{2}{|c|}{\multirow{1}{*}{\textit{\textbf{Type}}}}			&
\multicolumn{1}{c|}{\multirow{1}{*}{$d$}}							&
\multicolumn{1}{c|}{\multirow{1}{*}{$t$}}							&
\multicolumn{1}{c|}{\multirow{1}{*}{$\alpha$}}						&
%\multicolumn{1}{c||}{\multirow{1}{*}{$d^*$}}						&
\multicolumn{1}{c|}{\multirow{1}{*}{\textit{\textbf{Benchmarks}}}}	\\  \hline %\cline{1-3} %\hline

\multicolumn{1}{|c|}{\multirow{15}{*}{\textit{\textbf{St}}}}	&
\multicolumn{1}{c|}{\multirow{14}{*}{\textit{\textbf{D}}}}		&
\multicolumn{1}{c|}{\multirow{14}{*}{1}}		&
\multicolumn{1}{c|}{\multirow{4}{*}{0}}						&
       $1/2^{32}$		& BasicRSA-T\{100, 300\} \\ \cline{5-6}
       
&&&& 0.5 	& 	s15850-T100, s38584-T\{200, 300\} \\ \cline{5-6}
&&&& 0-0.25	&	wb\_conmax-T\{100, 200, 300\} \\ \cline{5-6}
&&&& 0-0.87	&	RS232-T\{100, 800, 1000, 1100, 1200, 1300, 1400, 1500, 1600, 1700, 1900, 2000\} \\ \cline{4-6}

&&& \multicolumn{1}{c|}{\multirow{3}{*}{1}}		&
	0.5	&	b15-T\{300,400\}								\\ \cline{5-6}
&&&& 0.5-0.75  &	s35932-T\{100, 200\}						\\ \cline{5-6}
&&&& 0-0.06	  &	RS232-T\{400, 500, 600, 700, 900, 901\} \\ \cline{4-6}

&&& \multicolumn{1}{c|}{\multirow{2}{*}{2}}		&
	0.5		&	vga-lcd-T100, b15-T\{100, 200\}				\\ \cline{5-6}
&&&& 0.87	&	 s38584-T100 							\\ \cline{4-6}

&&& \multicolumn{1}{c|}{\multirow{2}{*}{3}}		&
	$1/2^{32}$	&	BasicRSA-T\{200, 400\}				\\ \cline{5-6}
&&&& 0.5			&	s38417-T100 						\\ \cline{4-6}

&&& 5	&	0.99&	 s38417-T200  \\ \cline{4-6}
&&& 7	&	0.5	&	RS232-T300 \\ \cline{4-6}
&&& 8 	&	0.5	&	s35932-T300 \\ \cline{2-6}


%-----------------------------------------------------------------------------------------------------------------
												&
\multicolumn{1}{c|}{\textit{\textbf{ND}}}		&
\multicolumn{3}{c||}{ N/A }						&
MC8051-T\{200, 300, 400, 500, 600, 700, 800\}, PIC16F84-T\{100, 200, 300, 400\} \\ \hline

%-----------------------------------------------------------------------------------------------------------------
\multicolumn{2}{|c|}{\textit{\textbf{Si}}} 		& 
\multicolumn{3}{c||}{ N/A }						&
AES-T$\lbrace$400, 600, 700, 800, 900, 1000, 1100, 1200, 1300, 1400, 1500, 1600, 1700, 2000, 2100$\rbrace$, s38417-T300, AES-T$\lbrace$100, 200, 300$\rbrace$ \\ \hline 

\end{tabular}
%\vspace{-8pt}
\end{table}




%
%In order to provide concrete guarantees about which trojans can be detected by HaTCh under all circumstances and which ones can be detected under certain conditions, 
\tablename~\ref{table:trusthub_table} shows the relevant\footnote{Not all of the benchmarks from TrustHub are listed in \tablename~\ref{table:trusthub_table}, because some of them have no payload, such as RS232-T200. Similarly the payloads of some other benchmarks are harmless which would be removed by synthesis tools. E.g. RS232-T1800, which just adds three inverters to waste energy.} benchmarks from Trusthub categorized according to our framework.
\textit{St-D} group (i.e. $H_D$ Trojans) is further subdivided based on the properties ($d$, $t$, $\alpha$).
All these Trojans happen to be represented by a single trigger of dimension $d=1$ (i.e., the trigger is a single wire); whereas their corresponding $t$ and $\alpha$ values\footnote{$\alpha$ values show estimated upper bounds on probabilities.} are listed in \tablename~\ref{table:trusthub_table}.

To determine $t$ values of these trojans, we simply count the minimum number of registers between the trigger signal wires(s) and the output port of the IP core.
Since precisely calculating $\alpha$ can be almost impossible for large circuits, we estimate $\alpha$ values through experiments.
We argue that these estimated values closely represent the corresponding actual values of $\alpha$, hence \tablename~\ref{table:trusthub_table} fits the definition of $\alpha$.
In order to estimate $\alpha$ values, we first find the smallest chain of logic gates starting from the trigger signal wire(s) till the output port of the IP core (ignoring any registers in the path).
Then for each individual logic gate, we compute the probability of propagating a logic 1 (considering that the trigger wire(s) get a logic 1 upon a trigger event), e.g. an AND gate has the probability $1/4$ of propagating a logic 1, whereas an XOR gate has the probability $1/2$.
Finally we compute an aggregate probability of propagation by multiplying all the probabilities of each logic gate in the chain, which gives the value $1-\alpha$.
%This number provides a direct estimate of $\alpha$, since a higher number of logic levels means lower probability that the effect of the trigger signal activation will be seen at the output; hence it results in a higher $\alpha$ value.
%As explained earlier, the stealthiness factor $\alpha$ can be reduced by increasing $d$.
%In column $d^*$, \tablename~\ref{table:trusthub_table} shows the required minimum values of $d$ to have an estimated $\alpha=0$.
%It is worth mentioning that HaTCh is able to achieve $\alpha=0$ for these trojans by using locality of only $1$, i.e. $l=1$.
%HaTCh is able to detect all these \textit{St-D} trojans using $d=1$.

Notice that all these \textit{St-D} Trojans have a very low value of $d$ (particularly $d=1$) which reflects their low stealthiness, and hence the fact that these publicly available benchmarks represent only a small subset consisting of simple Trojans.
Even though some of these benchmarks have high values of $\alpha$ (e.g. s38584-T100 and s38417-T200), however in practice, having a very high value of $\alpha$ may not always be useful for the adversary.
Ideally, on one hand, the adversary wants the Trojan to be triggered in the logic testing phase only once, and remain undetected (i.e. by having high $\alpha$) so that the Trojan trigger is whitelisted.
On the other hand, after the testing phase, he wants the Trojan to deliver the payload by disrupting the normal output (i.e. by having low $\alpha$), otherwise the Trojan is not useful for him.
Therefore, the adversary would like to have a sweet spot between the high and low ends of $\alpha$ values.
%This essentially increases the chances for HaTCh to detect the trojan, i.e. either it gets detected (if triggered) in the learning phase (because $\alpha \ll 1$), or it gets detected by the tagging circuitry later.

%Table~\ref{table:trusthub_table} further subgroups \textit{St-D} trojans based on their payload propagation delay $t$, and it can be seen that $t$ is generally pretty small.
%All these trojans happen to have a trigger signal dimension $d=1$.
%Although HaTCh mainly focuses on trigger activated \textit{St-D} trojans, however it can also detect always-active \textit{St-D} trojans since such trojans are meant to always exhibit malicious behavior over the standard I/O channels which can be easily detected by functional testing during the learning phase.
%Notice, however, that always-active \textit{St-D} trojans are practically not useful for an adversary as they have no stealthiness.

%\subsubsection{ST-ND and Si Trojans}
\textit{St-ND}  (i.e. $H_{ND}$ group) and \textit{Si} Trojans are out of scope of this paper.
In our model, some TrustHub benchmarks, e.g. MC8051 series, are considered to be in $H_{ND}$ group because of their flexible design specifications.
The specification of a processor is relatively flexible about the timing/ordering of outputs (e.g. instructions execution) due to some unpredictable factors like interrupt requests etc. 
This flexibility, however, makes it harder for logic testing based tools to verify the functional correctness of the design. 
However, if there exists a precise and strict model for these cores, such HTs can still be analyzed in our model.
%Notice that trigger activated \textit{Si} trojans can actually be detected by HaTCh provided that these trojans do not get triggered during the HaTCh learning phase (so that their trigger related wires still remain blacklisted).
%\textit{Si} trojans exploit side channels to deliver the malicious payload and do not affect the normal functionality over standard I/O channels.
%If such a trojan gets activated during the learning phase, since HaTCh tool will not observe any malicious behavior on the standard I/O channels therefore it would whitelist the trigger related wires.
%On the other hand, if it does not get activated during the learning phase, only the non-malicious wires would be whitelisted and the trigger related wires would still remain in the blacklist leading to trojan detection.
%The same reasoning is applicable to \textit{TA-St-D-NF} trojans.
%Always-active \textit{Si} trojans, however, are out of the scope of HaTCh tool and cannot be detected.
%Since these trojans are not trigger-based, therefore they are always active during the learning phase.
%However such trojans always show malicious behavior in a way that does not harm the normal functionality of the IP core and hence HaTCh considers the circuitry as `normal' and whitelists it.






==> arxiv eprint/sections/introduction.tex <==
\section{Introduction} \label{sec:intro}

%\IEEEPARstart{M}{odern} 
Modern electronic systems heavily use third party IP (intellectual property) cores as their basic building blocks.
An IP core is a reusable block of logic, tailored to perform a particular operation in an efficient manner, that is an intellectual property of one party.
Optimized for area and performance, the IP cores are essential elements of design reuse in electronic design automation (EDA) industry and save a lot of resources to redesign the components from scratch. 
UARTs, DSP units, Ethernet controllers and PCI interfaces etc. are some examples of the IP cores~\cite{ipcore2}.

The IP cores are typically offered either in a hardware description language (e.g., Verilog or VHDL) as synthesizable RTL (also called `open source' IPs) or as generic gate-level netlists (also called `closed source' IPs).
These IP cores give rise to a critical security problem: how to make sure that the IP core does not contain a \textit{Hardware Trojan} (HT)?
A (compromised) IP core vendor acting as an adversary could implant a malicious circuitry in the IP core for privacy leakage or denial of service attacks.

A significant amount of research has been done during the past decade to design efficient tools for HT detection.
Hicks \textit{et al.}~\cite{sp2010} proposed \textit{Unused Circuit Identification} (UCI) which centers on the fact that the HT circuitry mostly remains inactive within a design, and hence such minimally used logic can be distinguished from the other parts of the circuit.
However later works~\cite{uci_1},~\cite{UCI_sp11} showed how to design HTs which can defeat the UCI detection scheme.
Zhang \textit{et al.}~\cite{veritrust} and Waksman \textit{et al.}~\cite{fanci} proposed detection schemes called VeriTrust and FANCI respectively and showed that they can detect all HTs from the TrustHub~\cite{trust_hub} benchmark suite.
Yet again, the most recent technique called DeTrust~\cite{detrust} introduces new Trojan designs which can evade both VeriTrust and FANCI.

The reason behind this cat-and-mouse game between attackers and defenders is that the current HT detection tools offer critically low HT coverage and typically only cover a small \textit{constant} set of \textit{publicly known} HT benchmarks such as TrustHub.
Whereas an adversary may design new HTs which are different from the publicly known HTs in that they can bypass the detection tool, as demonstrated by DeTrust~\cite{detrust}.
It is unclear to what extent the existing HT detection tools are effective for \textit{publicly unknown} HTs.

%\todo[inline]{Add importance of taxonomies in defining scope}

The first and foremost challenge in designing an effective HT detection technique is to define the scope of the countermeasure on the landscape of HTs.
The HT taxonomies can be used for this purpose.
Bhunia {\em et al.} \cite{ieeesurvey} presents a taxonomy of HTs
%, their general models and a taxonomy of the existing countermeasures 
based on an extensive survey of the existing literature.
The trigger based HTs are subdivided into digital and analog categories where digital HTs have two general models, combinational and sequential HTs.
Combinational HTs are those whose trigger circuitry is simply a comparator whereas sequential HTs have memory elements as well in their trigger circuitry.
Trojans are also classified based on payloads, i.e. digital, analog and others such as denial of service.
%Similarly, HT detection approaches are mainly divided into destructive and non-destructive approaches.
%Logic testing and side-channel analysis are the two major techniques under non-destructive approaches.

Since we are talking about digital IP cores, in this paper we limit ourselves to trigger activated digital HTs which have digital payloads. 
The Trojans that are always active and/or exploit side channels for their payloads are out of scope of this paper.


Even though existing HT taxonomies, such as the one mentioned above, provide significant knowledge about the HT properties, yet this information is quite fundamental and does not provide detailed characteristics vital for the HT countermeasures to provide strong security guarantees.
This limitation may lead to uncertainties and potentially misleading information about the detection coverage that a HT countermeasure can provide.

%This paper introduces of these detailed characteristics of trigger activated digital HTs is the key contribution of this paper which allows the HT detection techniques to provide transparent security guarantees.

%\subsection{Contributions}
This paper introduces four crucial properties ($d$, $t$, $\alpha$, $l$) of a large and complex class $H_D$ of trigger activated and deterministic digital HTs.
These properties, determining the stealthiness of HTs, lead to a much more detailed classification of such HTs and hence assign well defined boundaries to the scope of the existing and new countermeasures on the huge landscape of HTs.
In our model, $H_D$ represents the HTs which are embedded in a digital IP core whose output is a function of only its input, and the algorithmic specification of the IP core can exactly predict the IP core behavior.
A brief highlight of the properties of $H_D$ is as follows:

{
\vspace{6pt}
\renewcommand{\arraystretch}{1.3}
\centering
\begin{tabular}{c p{0.85\columnwidth}} %\hline
$d$: &  \textbf{Trigger Signal Dimension} represents the number of wires used by HT trigger circuitry to activate the payload circuitry in order to exhibit malicious behavior. Large $d$ shows a complicated trigger signal, hence harder to detect. \\ %\hline
$t$: & \textbf{Payload Propagation Delay} is the number of cycles required to propagate malicious behavior to the output port \textit{after} the HT is triggered. Large $t$ means it takes a long time after triggering until the malicious behavior is seen, hence less likely to be detected during testing. \\ %\hline
$\alpha$: & \textbf{Implicit Behavior Factor} represents the probability that given a HT gets triggered, it will not (explicitly) manifest malicious behavior; this behavior is termed as implicit malicious behavior. Higher probability of implicit malicious behavior means higher stealthiness. \\ %\hline
$l$:  & \textbf{Trigger Signal Locality} shows the spread of trigger signal wires of the HT across the IP core. Small $l$ shows that these wires are in the close vicinity of each other. Large $l$ means that these wires are spread out in the circuit, hence the HT is harder to detect. \\ %\hline
\end{tabular}
\vspace{3pt}
}


%\subsubsection{Stealthiness due to the IP Core Behavior}
%Notice that not only the trojan itself, but also the IP core in which it has been embedded plays a major role in its stealthiness.
%For example, a trigger based trojan with a digital payload of producing incorrect result embedded in a multiply-accumulate core could be detected by logic testing.
%But it might not be possible to detect it in a random number generator core through logic testing, as normal and malicious behaviors might be indistinguishable because of the inherent non-determinism of the core.
%For example, the incorrect behavior produced by a trojan may not always propagate to the output, or if it does it might not be distinguishable from an otherwise normal output because of the nature of the IP core; and hence go undetected by logic testing.
%The existing trojan taxonomies only talk about the basic trojan properties, and do not consider the added stealthiness because of the IP core behavior.
%This effect also needs to be incorporated to classify hardware trojans in much more detail.

%\subsubsection{Weak Security Guarantees}
%Since the existing classifications of trojans are quite general and do not have much detailed differentiation of trojans, the existing countermeasures cannot provide strong security guarantees for any of these classes of trojans because their scope is not well defined.
%In other words, these countermeasures may see `false negatives'.
%However notice that without a well defined scope of a countermeasure, its false negatives rate provides misleading information about the effectiveness of the tool because the observed false negatives could be the result of out-of-scope trojans.
%If the scope of a particular countermeasure is well defined through a comprehensive and detailed taxonomy, it can provide strong security guarantees within its scope.

Based on the above mentioned parameters, we introduce a new stealthy HT, coined the \textit{XOR-LFSR}, which cannot be efficiently detected by ordinary means (design knowledge of the HT itself needs to be incorporated in the detection tool).
%By incorporating the knowledge and understanding of these parameters, HT detection schemes can detect orders of magnitude larger HT subclasses.
%We demonstrate that logic testing based traditional HT detection tools can be bypassed by ``stealthy'' HTs (e.g., those with a large $d$ value) and 
We also show that the current publicly known HTs have small $d$ (mostly $d=1$ for TrustHub) and hence they are the simplest ones.
\figurename~\ref{fig-coverage} depicts a pictorial representation of the HT class $H_D$ that includes TrustHub\footnote{In this paper, we are only considering HTs from TrustHub that are trigger activated and have digital payloads.}.
Although VeriTrust and FANCI can detect TrustHub HTs, it is unclear what security guarantees they offer outside TrustHub.

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{coverage}
\caption{Class of Deterministic Hardware Trojans $H_D$, and detection coverages of existing Hardware Trojan countermeasures.}
\label{fig-coverage}
\end{figure}




%\vspace{3pt}
%\textbf{HaTCh Methodology: }
%%The HaTCh tool takes the type of trojan to detect as input in the form of parameters $t$, $\alpha$ and $d$, and detects all such trojans in polynomial time complexity.
%Our proposed HT detection tool HaTCh works in two phases; a \textit{learning phase} and a \textit{tagging phase}.
%The learning phase performs logic testing on the IP core and produces a blacklist of all the unactivated (and potentially untrusted) transitions of internal wires.
%The tagging phase adds additional logic to the IP core to track these untrusted transitions.
%HaTCh also allows the user to control the desired security level and false positives rate. 
%We have implemented HaTCh and our experimental as well as theoretical results demonstrate that:
%\begin{itemize}
%\item HaTCh detects all $H_D$ trojans in $poly(n)$ time where $n$ is number of circuit wires and the degree of the polynomial corresponds to the stealthiness of the HT embedded in the circuit. In particular, all $H_D$ trojans from TrustHub are detected in linear time.
%\item HaTCh incurs low area overhead (on average $4.18\%$ for a set of tested HT benchmarks).
%\item In cases where state of the art HT detection tools have a worst case exponential complexity in the number of circuit inputs, HaTCh offers orders of magnitude lower complexity.
%\end{itemize}




%Therefore, a rigorous security framework of HTs should characterize the potentially \textit{exponentially large} class of HTs from which HTs can be detected (with possibly an exponential amount of work) with negligible false negative rate.
%The detection tools should then be evaluated based on the subclass of HTs that they can detect with acceptable performance overhead.
%their efficiency in combination with their ability to detect \textit{any} trojan from this huge class.

%Current state of the art HT detection schemes include extensions of VeriTrust and FANCI, proposed by \cite{detrust}, which enable them to detect somewhat larger subclasses of HTs.
%The admitted limitation of these techniques is their insanely high computational complexity for medium to large sized circuits.
%\figurename~\ref{fig-pre_complexities} compares the computational complexities of extensions of VeriTrust/FANCI with HaTCh to detect a simple $m$-input AND gate type HT.
%We show in section~\ref{sec:hatch_framework} that HaTCh offers sub-exponential complexity as opposed to the exponential complexity of VeriTrust/FANCI.

%Additionally, VeriTrust and many other existing logic testing based HT detection schemes implicitly assume that a HT is either not triggered during the testing phase, or if it does get triggered then it is \textit{always} detected because it produces incorrect output.
%Surprisingly, there is also a third possibility, i.e. a HT gets triggered during the testing phase yet it does not produce any incorrect output and hence remains undetected.
%This behavior, termed as \textit{implicit malicious behavior}, leads to serious security vulnerabilities in the current state of the art HT detection schemes such as VeriTrust and extended VeriTrust.
%We show how an adversary can bypass such detection techniques by exploiting implicit malicious behavior.



% *******************************
% FP & FN Table and Complexity Figure
% *******************************

%\begin{table}[!t]
%\renewcommand{\arraystretch}{1.4}
%\caption{Comparison of False Negatives and False Positives of Hardware Trojan countermeasures for $H_{t,d,\alpha}$.}
%\label{table:false_pos_neg_comparison}
%\centering
%%\begin{tabular}{ | m{2.5cm} | m{0.7cm} | m{1cm} | m{1cm}| m{1cm} | m{1cm}|}
%\begin{tabular}{ | c || m{2.2cm} | c |}
%\hline
%
%    & \textbf{VeriTrust/FANCI} & \textbf{HaTCh} \\ \hline
%    \textit{\textbf{False Negatives}}  & Unknown Characterization & Controllable. $2^{-\lambda}$ for $H_{t,d,\alpha}$ \\ \hline
%    \textit{\textbf{False Positives }} & Uncontrollable &  Controllable. $\rho$ for $H_{t,d,\alpha}$ \\ \hline
%
%\end{tabular}
%%\vspace{-10pt}
%\end{table}
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.99\columnwidth]{pre_complexities}
%\caption{Comparison of pre-silicon phase computational complexities of Hardware Trojan countermeasures.}
%\label{fig-pre_complexities}
%\end{figure}


%==================================================================
% Started bulk commenting below %

%\subsection{Contributions}
%In this paper, we present a rigorous framework called \textit{\textbf{Ha}rdware \textbf{T}rojan \textbf{C}atc\textbf{h}er} (HaTCh) for HT design and detection.
%We assume an adversarial model where the IP core is closed source.
%Hence, the IP core vendor only provides the generic gate level netlist of the IP core, and its functional specifications in the form of a polynomial time algorithm which can be used to verify the I/O behavior of the core.
%In order for an adversary to be able to access embedded HTs in millions of fabricated chips, we assume in this paper only remote adversaries who do not have physical access to exploitable side channels.\footnote{First, physical presence is not a scalable option for being able to attack (a large subset out of) millions of chips. Second, the timing side channel is the only side channel accessible by a remote adversary: we assume that Internet connections add too much timing noise to make use of such channels. HTs in processors may make use of the cache side channel, which we regard in our framework as a covert channel that can be detected by a logic testing based tool (in Definition \ref{def:htp}) as a spec violation of execution times.}
%The key contributions of the HaTCh framework are as follows:
%
%\vspace{3pt}
%\textbf{Characterization of HTs:}
%We first differentiate two groups of IP cores with HTs that do not exploit side channels; $H_D$ and $H_{ND}$.
%For HTs $\in H_D$ the IP core expresses deterministic (non-probabilistic) functionality and the IP core spec can be used to verify this functionality.
%% (in particular, most IP cores that implement security critical primitives have this deterministic property).
%We note, if an IP core $\in H_{ND}$, i.e. its specification allows probabilistic fluctuations in the output (a covert channel is possible), then a logic testing based tool cannot detect a HT which embeds information at a non-negligible rate within those fluctuations (e.g. by using watermarking techniques).
%%This implies that HT detection problem for $H_{ND}$ has no solution.
%
%\vspace{3pt}
%\textbf{HT Design Parameters:} 
%For the deterministic group $H_D$, we introduce certain crucial design parameters ($t$, $\alpha$, $d$, $l$) of HTs which determine the stealthiness of a HT.
%The impact of having large values of these HT parameters is briefly as follows:
%{
%\vspace{3pt}
%\renewcommand{\arraystretch}{1.0}
%\centering
%\begin{tabular}{c p{2.8in}} %\hline
%$d$: & Complicated trigger signal, harder to detect. \\ %\hline
%$t$: & Long time until payload triggers, less likely to be detected during testing. \\ %\hline
%$\alpha$: & Higher probability of implicit malicious behavior, higher stealthiness. \\ %\hline
%$l$:  & Weak locality, trigger wires spread out in the circuit, harder to detect. \\ %\hline
%\end{tabular}
%\vspace{3pt}
%}
%%By incorporating the knowledge and understanding of these parameters, HT detection schemes can detect orders of magnitude larger HT subclasses.
%We demonstrate that logic testing based traditional HT detection tools can be bypassed by ``stealthy'' HTs (e.g., those with a large $d$ value) and we show that currently benchmarked HTs (having small $d$) are the simplest ones in the huge HT landscape, and hence represent just the tip of the iceberg. 
%Based on these parameters, we introduce a new stealthy HT, coined the \textit{XOR-LFSR} trojan, which cannot be efficiently detected by ordinary means (design knowledge of the HT itself needs to be incorporated in the detection tool).
%
%\vspace{3pt}
%\textbf{HT Detection Tool:}
%We present a powerful HT detection tool for group $H_D$ which solves the following precise HT detection problem:
%
%\begin{definition} \label{def:htp}
%\textit{HT Detection Problem:}
%Design a logic testing based detection algorithm (tool) for $H_D$ which takes the following inputs:
%\begin{itemize}
%\item IP core netlist \& functional specifications.
%\item Security parameter $\lambda$
%\item Maximum acceptable false positive rate $\rho$
%\end{itemize}
%
%and produces the description of additional (tagging) circuitry to be added to the IP core which offers:
%\begin{itemize}
%\item Malicious behavior detection probability $1-negl(\lambda)$
%\item A false positive rate $\le \rho$
%\item Area overhead polynomial in the IP core size
%\end{itemize}
%
%\end{definition}
%
%We show in section \ref{sec:hatch_framework} that the HT detection problem for $H_D$ can be solved:
%%On the other hand, our proposed detection tool can detect \textit{any} trojan in $H_D$.
%Let $n$ be the number of wires in an IP core (which is potentially infected by a HT), and let $\rho$ be the maximum acceptable false positive rate of a HT detection tool, then 
%%we prove the following theorem in section \ref{sec:hatch_framework} for HaTCh's computational complexity:
%
%\begin{theorem} \label{th:complexity}
%There exists a tool, coined HaTCh, that solves the HT detection problem for the set of HTs $\in H_D$ corresponding to fixed parameters ($t$, $\alpha$, $d$). 
%The computational complexity of HaTCh is $O\left( \frac{\lambda}{\log_2(1/\alpha)} \cdot \frac{(2n^2)^{d}}{\rho} \right)$ 
%(polynomial in the IP core size $n$). % and is inversely proportional to the maximum acceptable false positive rate $\rho$.
%\end{theorem}


% till here 
%==================================================================



The rest of this paper is organized as follows.
Section \ref{sec:background-org} provides some basic background of HTs and introduces our threat model.
Section \ref{sec:classification} defines the HT class $H_D$ and introduces several advanced properties of this class which lead to new HT design methodologies.
%Sections \ref{sec:hatch_algo} and \ref{sec:hatch_framework} present the basic algorithm and the detailed implementation of HaTCh respectively.
%In section \ref{sec:comparisons} we compare HaTCh with state of the art HT detection schemes.
%Section \ref{sec:evaluation} shows the experimental evaluation.
%Related work is presented in section \ref{sec:related_work} and we finally conclude in section \ref{sec:conclusion}.




==> arxiv eprint/sections/related_work.tex <==
\vspace{6pt}
\section{Related Work}\label{sec:related_work}

Hardware trojans have recently gained significant interest in the security community~\cite{taxonomy},~\cite{usenix08},~\cite{huntforkill}. 
The works~\cite{usenix08} and~\cite{huntforkill} showed how malicious entities can exist in hardware, while Skorobogatov \emph{et al.}~\cite{military} showed evidence of such backdoors in military grade devices.
Nefarious designs have also been deployed and detected in wireless communications devices~\cite{wireless}.
Recent works have mostly focused on detection~\cite{iccd_12} and identification schemes~\cite{iccad_12}, which assess to what extent the pieces of hardware may be vulnerable, and how related trojans can be classified.
State of the art HT detection schemes include UCI~\cite{sp2010}, VeriTrust~\cite{veritrust}, FANCI~\cite{fanci} and DeTrust~\cite{detrust}.
Typically, HT detection techniques only show their detection capabilities for HTs from the TrustHub benchmarks suite, in which all trojans are explicitly triggered.
This explicitness forgoes the lack of implicitness, due to which all the above schemes are able to detect the benchmarked trojans.
These schemes, however, do not cater for higher dimensional ($d>1$) trojans or the added stealthiness because of the implicit malicious behaviors (i.e. $\alpha$).
DeTrust presents a trojan example which bypasses other existing countermeasures, and interestingly it happens to have the dimension $d=2$.
However, this property has not been noticed or analyzed in that paper.
We fill these gaps by providing a detailed and rigorous framework to reason about HT characteristics and their impact on the detection schemes.
%% *************************************************************** 


%\vspace{6pt}
%\textbf{Side-Channel HT Detection Techniques:} 
Further works construct and detect HTs that use side channels~\cite{sidechannel1, sidechannel2, sidechannel3}.
Such HTs remain implicitly on, and have usually no effect on the normal functionality of the circuit.
Side channels include power based channels~\cite{power2}, as well as heat based channels~\cite{power4}.
Power based HTs force the circuit to dissipate more and more power to either damage the circuit, or simply waste energy.
Heat based HTs leak important information via heat maps~\cite{heat}, where highs and lows in heat dissipation can be interpreted as logic 1's and 0's.
%The above works seem to be complete in the sense that the threat model contains side channel vulnerabilities, however, this paper uses threat models that cater for direct contacts between the user and the design.
Our work only focuses on HTs that perturb standard I/O channels; analyzing side channel models/frameworks is out of scope of this paper.
%The presence of a non-zero false negative rate in an adversarial model that allows side channel HTs implies a constant rate of privacy leakage.%\footnote{Therefore, as a design principle, IP cores that need to protect against (maliciously engineered) leakage over side channels must implement leakage resilient key renewal, e.g., as described in \cite{hazay2013leakage}.
%It is outside the scope of this paper to analyze side-channel models/frameworks in existing literature that may lead to tools that can detect side channel HTs with small false negative rates or obfuscate (by adding extra circuitry) the effect of such HTs leading to reduced privacy leakage rates.


==> arxiv eprint/sections/trojan_class.tex <==
\section{Characterization of Hardware Trojans}\label{sec:classification}

\begin{figure}[!t]
\centering
\includegraphics[width=0.9\columnwidth]{taxonomy} 
%\vspace{-18pt}
\caption{Classification of Hardware Trojans}
\label{fig:taxonomy}
%\vspace{-12pt}
\end{figure}

%Now that we have explained some important terminologies related to HTs which we will be using frequently in the rest of the paper, 
In this section, we characterize the trigger activated HTs based on their following fundamental characteristics that lead to a clear distinction between the deterministic $H_D$ and non-deterministic $H_{ND}$ types.


% ---------------  Standard Channels vs. Side Channels  ----------------------------
\subsection{$St$ vs. $Si$ Hardware Trojans} 
Hardware Trojans are first grouped based on the payload channels they use once activated as shown in  \figurename~\ref{fig:taxonomy}.
\textit{St} refers to the Trojans using only standard I/O channels (this includes LED outputs etc.) whereas \textit{Si} represents the Trojans which also use side channels to deliver the payload.
I/O channels are generally used to communicate binary payloads $b_j$ at certain times $t_j$ for the duration of the execution of the IP core. 
In this sense the view of an I/O channel can be represented as a sequence $(b_1,t_1), (b_2,t_2),\ldots, (b_N,t_N)$. 
Its information is decomposed in three channels: the binary channel corresponding to $(b_1, b_2, \ldots, b_N)$, the timing channel corresponding to $(t_1,t_2,\ldots, t_N)$, and the termination channel $N$ which reveals information about the duration of the execution of the IP core. 
If a Trojan delivers some of its payload over the timing channel (or other side channels), then we define it to be in \textit{Si}. 
If a Trojan delivers {\em all} of its payload using the standard usage of  I/O channels (the binary and termination channels), then we define it to be in \textit{St}.  
E.g., a HT causing performance degradation in terms of slower response/termination times due to slower computation (denial of service in the most extreme case) is in \textit{St}.



% ----------------- Deterministic vs. Non-deterministic IP Core / Specifications ----------------------
\subsection{$H_D$ vs. $H_{ND}$ Hardware Trojans} 
We further refine our description of \textit{St} Trojans by subdividing them in $H_D$ and $H_{ND}$ groups based on the IP core behavior in which they are embedded and their algorithmic specifications.

\begin{definition}
\boldmath{$H_D$} Trojans are the ones which are:
\begin{enumerate} 
\item Embedded in an IP core whose output is a function of only its input -- i.e. the logical functionality of the IP core is deterministic, and 
\item The algorithmic specification of the IP core can exactly predict the IP core behavior.
\end{enumerate}
\end{definition}

If any of the two above mentioned conditions is not satisfied for a \textit{St} type HT then we consider the HT to be in $H_{ND}$.
A true random number generator (TRNG), for example, is a non-deterministic IP core since its output cannot be predicted and verified by logic testing against an expected output.\footnote{Any IP core which contains a TRNG as a module, yet the I/O behavior of the core can still be predicted is considered $H_D$.}
Any \textit{St} Trojan in such a core is considered $H_{ND}$.
A pseudo random number generator (PRNG), on the other hand, is considered a deterministic IP core as its output depends upon the initial seed and is therefore predictable by a logic based testing tool (hence $H_D$).
Similarly, if the algorithmic specification allows coin flips generated by a TRNG then we consider the Trojan to be $H_{ND}$.
On the other hand, if the coin flips are generated by a PRNG then we regard the Trojan as $H_D$.

The non-deterministic behavior of IP cores and/or their functional specification which accepts small probabilistic fluctuations within some acceptable range allows a covert channel for $H_{ND}$ Trojans to embed some minimal malicious payload in the standard output without being detected by an external observer~\cite{bellare2014security}.
The external observer considers these small fluctuations as part of the functional specification.
Hence, the non-deterministic nature of $H_{ND}$ Trojans prohibits the development of a logic testing based tool to detect these Trojans with overwhelming probability.



% *************************************************
% ElGamal EXAMPLE
% *************************************************
%E.g.,  the probabilistic ElGamal signature scheme produces signatures of the form $(r,s)$ where $r=g^k$ and $s=(H(m)-x\cdot (g^k \mod p))k^{-1} \mod (p-1)$, where $k\in \{1,\ldots,p-1\}$ is random with $gcd(k,p-1)=1$, can be exploited by a hardware Trojan in $H_{ND}$ if $k$ is extracted from a TRNG. 
%The secret key $x$  can be leaked as follows. The Trojan implements a secret pseudo random permutation $R$ only known to the adversary. 
%The Trojan keeps a counter and for the $i$-th encryption it simply produces a random $k$ with  $gcd(k,p-1)=1$  among those $k$ for which the least significant bit in $R(r,s)$ is equal to the $(i \mod |x|$)-th bit in the binary representation of $x$, hence, an adversary who eavesdrops a consecutive sequence of signatures is able to extract $x$. 
%A legitimate user cannot see any deviation form ElGamal's functional specification (and even if the user suspects an attack of this kind, it cannot be detected by using the signature and secret key because of  the pseudo random permutation $R$).   
%If $k$ is generated by a PRNG, then its seed can be set/programmed and logic testing (as done in HaTCh) can verify produced signatures  to correspond to correct pseudo random numbers (which are not generated by a Trojan). 

% *************************************************


%[TO DO: what about probabilistic encryption using a TRNG -- can the random numbers be recovered and embed a covert channel? If so, one should use a pseudo random number generator in such primitives.] 

%\begin{proof}[of Theorem \ref{th:non-deter}]
%Consider a finite state machine (FSM) having $k$ possible states $\{S_0, S_1, \dots S_{k-1}\}$ and an output associated with each state $\{y_0, y_1, \dots y_{k-1}\} \in R$ where $R$ represents an integer interval $[a,b]$ (for simplicity, we consider Moore state machine where the output only depends on the state).
%The FSM makes a state transition every clock cycle (without requiring any input, for simplicity).
%To introduce non-determinism in the FSM, suppose that state transitions are probabilistic where $p_{i,j}$ denotes the probability of transition from a current state $S_i$ to the next state $S_j$.
%Because of probabilistic state transition, the output $y_j$ as a result of transition to state $S_j$ is non-deterministic, yet within the acceptable range $R$.
%Let the output is sampled by an external observer after every $w$ clock cycles window and $w$ is large enough such that the outputs $y_i$ and $y_{i+1}$ sampled in $i_{th}$ and $(i+1)_{th}$ time window are uncorrelated, or in other words independent.
%Notice that the normal specification of this IP core only requires the output $y_i$ to be in the interval $R$, i.e., $y_i \in R$ in order to pass the logic testing.
%
%Let there is a hardware Trojan in this core which intends to leak some secret bit(s) $\delta=\{ \pm 1\}$ without violating the specifications.
%The Trojan modifies the output $y_i$ to $y'_i$ to embed the secret information into it as follows:
%\begin{equation} \label{eq:SecretTrojanExample}
%y'_i = \left\{
%	\begin{aligned}
%	& y_i + \delta & \text{if } (y_i + \delta) \in R \\
%	& y_i 		&\text{otherwise}
%	\end{aligned} \right.
%\end{equation}
%In other words, the Trojan introduces a bias in the output, while not violating the specifications, which shifts the expected \textit{mean} value $\mu$ of the `Trojan-free' core to $\mu' > \mu$ (for $\delta=+1$) or $\mu' < \mu$ (for $\delta=-1$).
%According to the law of large numbers, for a significantly large number $N$,  the average $\overline{y'_i}=\frac{1}{N}(y'_1 + y'_2 + \dots + y'_N)$ of $N$ independent (uncorrelated because of large time window $w$) output samples $y'_i$ approaches to $\mu'$, i.e., $\overline{y'} \rightarrow \mu'$.
%Hence, by computing the average $\overline{y'_i}$, the adversary can determine the secret $\delta$ as follows: 
%\begin{equation*}
%\delta = \left\{
%	\begin{aligned}
%	& +1 	& \text{if } \overline{y'_i} > (\mu+\tau) \\
%	& -1 	& \text{if } \overline{y'_i} < (\mu-\tau)
%	\end{aligned} \right.
%\end{equation*}
%where $\tau$ represents a small noise margin.
%Notice that the Trojan can be designed to leak several bits, over a long period of time, simply by embedding a new $\delta$ in (\ref{eq:SecretTrojanExample}) after $N$ time windows.
%The adversary, having the knowledge of $N$, can determine the leaked bits one by one after the initial synchronization.
%\end{proof}


\section{Advanced Properties of Class $H_D$} \label{sec:HD}

In the following discussion, we introduce some crucial properties of $H_D$ Trojans that characterize their complexity and stealthiness.

\subsection{Trigger Signal Dimension $d$}
When a trigger condition of a hardware Trojan occurs, {\em regardless of the other subsequent user interactions}, its trigger circuitry gets activated and outputs a certain binary value on a certain trigger signal $Trig$ to activate the payload circuitry which manifests malicious behavior.
A trigger signal $Trig$ is represented as a labeled binary vector of one or more wires/registers/flip-flops (each carrying a $0$ or $1$), e.g. in the example circuit of \figurename~\ref{fig:simple_ht_example}, $Sel=1$ is a trigger signal.
In other words, $Trig$ represents a trigger state of the circuit through which the circuit must have passed before manifesting malicious behavior.
Notice that the trigger state(s) can be associated back to the occurrence of the respective trigger condition(s).
Hence a HT can be represented by a set of trigger states ${\cal T}$; i.e. the states which always lead to malicious behavior (implicit or explicit).
\begin{definition} 
\textbf{A set \boldmath{${\cal T}$} of trigger states} \textit{represents} a HT if the HT always passes through one of the states in ${\cal T}$ in order to express implicit of explicit malicious behavior.
\end{definition}

\vspace{3pt}
Notice that {${\cal T}$} is not unique. 
For example, {${\cal T}$} could be {${\cal T} = \{(Sel=1)\}$}, or if $Sel$ is somehow independent of $A$ and $B$, then it could also be {${\cal T}=\{[(A,B)=(1,1)], [(A,B)=(0,0)]\}$} etc.

We define the \textit{trigger signal dimension} $d$ of a HT represented by a set of trigger states ${\cal T}$ as follows:
\begin{definition} 
\textbf{Trigger Signal Dimension \boldmath{$d({\cal T})$}} of a HT is defined as $d({\cal T}) = \max_{Trig \in {\cal T}} |Trig|$.
\end{definition}

\vspace{3pt}
In other words, the trigger signal dimension shows the width of the widest trigger signal bit-vector of a HT.
E.g. for the HT from \figurename~\ref{fig:simple_ht_exp_2}, $d({\cal T})=1$ since the set of trigger states {${\cal T} = \{(Sel=1)\}$} only has the signal $Sel$ that activates the payload circuitry is only 1-bit wide (and hence easy to detect).
In the next section, we show that one can design HTs with high dimensional trigger signals.
%A set of trigger states ${\cal T}$ {\em represents} the hardware Trojan if any of its malicious behaviors must have (at some clock cycle) passed through a state in ${\cal T}$. 
%The dimension of a set of trigger states ${\cal T}$ is defined as $d({\cal T}) =  \max_{Trig \in {\cal T}} |Trig|$. % and 
%Let ${\bf T}$ denote the collection of all possible sets ${\cal 
 % i.e. $Trig\in \{0,1\}^d$, and we call $d$ 
 %  the dimension of a Trojan is defined as 
%  the maximum width of a trigger signal , i.e.
%   $d=\min_{{\cal T}} w({\cal T}) $ where the minimization is over all possible sets ${\cal T}$ of trigger signals that represent the Trojan.
   %(which we also call trigger states) through which malicious behavior must transition.
Obviously, it becomes difficult to detect HTs which only have high dimensional sets of trigger states, i.e. large trigger signals.
The set of possible values of a given trigger signal $Trig$ grows exponentially in $d=|Trig|$ and only one value out of this set can be related to the occurrence of the corresponding trigger condition. 
Clearly, since in theory $d$ can be as large as the number of wires $n$ in the IP core, $H_D$ represents an exponentially (in $n$) large class of possible HTs.

\subsection{Payload Propagation Delay $t$}
For a set ${\cal T}$ which represents a HT, we know that if the HT manifests malicious behavior, then it must have transitioned through a trigger state $Trig\in {\cal T}$ at some previous clock cycle. 
Therefore, we define the \textit{payload propagation delay} $t$ as follows:
\begin{definition}
\textbf{Payload Propagation Delay \boldmath{$t({\cal T})$}} of a hardware Trojan represented by a set of trigger states ${\cal T}$ is defined as the {\em maximum} number of clock cycles taken to propagate the malicious behavior to the output \textit{after} entering a trigger state in ${\cal T}$. 
\end{definition}
%A $H_D$ Trojan that manifests malicious behavior % (consider the explicit malicious behavior for now) 
%must have first seen its \textit{trigger condition} occurring and transitioned through a trigger state $Trig$ from a set of trigger signals ${\cal T}$ which  represents the Trojan. We define  ....... [TO DO]
% of ``no return'' (which we have called a trigger state). 
%Clearly, since the number of possible states is finite, there must be some upper bound $t$ on the number of cycles within which malicious behavior manifests after a ``last trigger state''.
%In other words, $t$ represents the number of clock cycles taken to propagate the malicious behavior of a Trojan to the output port \textit{after} a trigger condition (corresponding to the last state  has occurred, i.e. from the moment when a trigger condition occurs till the moment when its resulting malicious behavior shows up at  the output port.
%For simplicity, we considered only explicit malicious behavior so far; however, the same logic applies to the Trojans with implicit malicious behavior as well.
%Such Trojans also see a trigger condition and then propagate some (malicious) result to the output; although this result happens to be the same as `normal' or `expected' result.
%The definition of $t$ can be further clarified with the following example.

I.e., the number of clock cycles from the moment when a trigger signal is asserted till its resulting malicious behavior shows up at the output port.
E.g., consider a counter-based HT where malicious behavior immediately (during the same clock cycle) appears at the output as soon as a counter reaches a specific value. 
Then, $t(\{Trig\})=0$ for the trigger signal $Trig$ which represents the occurrence of the specific counter value (i.e. trigger condition).
However, notice that any counter value $j$ clock cycles before reaching the `specific value' can also be considered as a trigger signal $Trig$ with $t(\{Trig\})=j$, because eventually after $j$ cycles this $Trig$ manifests the malicious behavior.
%On the other hand if we consider the trigger signal $Trig$ which represents the counter value $j$ clock cycles before reaching the specific value, then $t(\{Trig\})=i$.
%
%trigger condition is that the counter reaches a specific value. 
%In this case, $t$ is the latency between the moment when the counter reaches that specific value (the trigger condition) and the moment when its resulting malicious behavior appears at the output. 
%Note that $t$ is independent of the cycles required by the counter to reach the trigger condition and $t$ is 

To detect a HT with a large value of $t({\cal T })$, the memory requirement and complexity of logic testing based detection tool is increased.
However, for any HT, typically there exists a set of trigger signals which represents the HT and which has a small $t$ because of a small number of register(s) between the trigger signal and the output port.

%For the $k$\textit{-XOR-LFSR} Trojan in \figurename~\ref{fig-htd}, $t=0$ since the output is changed in the same clock cycle in which the Trojan gets triggered.

\subsection{Implicit Behavior Factor $\alpha$}
In addition to previously discussed properties of Trojans, the IP core in which the Trojan is embedded plays a critical role in its stealthiness.
According to the definition of implicit malicious behavior, it may not always be possible to distinguish a malicious output from a normal output just by monitoring the output ports.
Consequently, the implicit malicious behavior adds to the stealthiness of the HT since it creates a possibility of having a false negative under logic testing based techniques.
%For example, consider a Trojan being a malicious 2-to-1 MUX, with one of its inputs connected to a malicious wire and the other one to a normal wire (as  in \figurename~\ref{fig:simple_ht_example}). 
%Suppose  the Trojan  triggers and selects as a result the malicious wire as the MUX output instead of the normal wire. If the normal and malicious input have the same value, then the`malicious' output value is indistinguishable from the normal output value.
%Similarly, hardware Trojans embedded in non-deterministic IP cores can also produce such malicious outputs which seem to be legitimate because of inherent randomness of such IP cores.
We quantify this possibility by defining the \textit{implicit behavior factor} $\alpha$ as follows:
%\begin{definition}
%\label{def:aplha}
%\textbf{Implicit Behavior Factor \boldmath{$\alpha({\cal T})$}} of a HT represented by the set of trigger states ${\cal T}$ is defined as 
%$\alpha({\cal T}) = \underset{Trig\in {\cal T}}{\max} \alpha(Trig)$ where $\alpha(Trig)$ shows the probability that, given the trigger state $Trig$ occurs, it will lead to {\em implicit} malicious behavior.
%\end{definition}
\begin{definition}
\label{def:aplha}
\textbf{Implicit Behavior Factor \boldmath{$\alpha({\cal T})$}} of a HT is the probability that given the HT is triggered, it will manifest {\em implicit} malicious behavior.
\end{definition}
%The effect of the IP core on the stealthiness of a hardware Trojan (which is embedded into it) against logic testing techniques can be represented by the stealthiness factor $\alpha$: For a trigger state $Trig$ we define $\alpha(Trig)$ as the probability given that $Trig$ occurs, this will lead to  {\em implicit} malicious behavior.
%We define $\alpha({\cal T})$ as the {\em maximum} of $\alpha(Trig)$ over $Trig\in {\cal T}$.
% probability that given a trigger state in ${\cal T}$, the Trojan manifests an implicit malicious behavior (which can go undetected by the functional testing), i.e.
%\begin{equation*} \alpha = Prob(Implicit Malicious Behavior | Trigger Occurs) \end{equation*}

In other words, the higher the value of $\alpha$, the lower the chance of detection by logic testing even if the HT gets triggered and hence the higher the overall stealthiness of the HT.
E.g. for the HT from \figurename~\ref{fig:simple_ht_exp_2} with the trigger condition $A=B$, if $(A,B)=(1,1)$ then the malicious output $S=1$ is distinguishable from the normal output (i.e. $S=0$).
However for $(A,B)=(0,0)$, the malicious\footnote{The output is considered malicious because it is generated by an activated hardware Trojan.} output $S=0$ is indistinguishable from the normal output (i.e. $S=0$), i.e. the implicit malicious behavior comes into the picture.
Hence, given that this particular HT activates, the probability that the HT-generated (malicious) output is indistinguishable from the normal output is $\alpha({\cal T}) = 0.5$ which represents the implicit behavior factor of this HT.

%\subsubsection{Notation used for $H_D$ Trojans: $H_{t,\alpha,d}$}
%\begin{figure}[!t]
%\centering
%\includegraphics[width=\columnwidth]{achievable}
%\caption{Effects of changing the parameters $t$ and $d$ on $\alpha$.}
%\label{fig:alpha_tradeoffs}
%\end{figure}



%****************** Locality 
\subsection{Trigger Signal Locality $l$}

\begin{figure}[!t]
\centering
\subfloat[A simple circuit]{\includegraphics[width=2in]{locality_circuit}
\label{fig:locality_circuit}}
\hfil
\subfloat[Locality Graph of the circuit]{\includegraphics[width=2in]{locality_graph}
\label{fig:locality_graph}}
\caption{Example of Locality Graph}
\label{fig:locality_graph_example}
\end{figure}

We notice that the individual wires of a HT trigger signal of dimension $d$ are logically/physically located in the close vicinity of each other in the circuit netlist/layout.
This is because eventually these wires need to coordinate (through some combinational logic) with each other to perform the malicious operation.
Based on this observation, we introduce the idea of \textit{locality} in gate level circuits, similar to the region based approach in \cite{trustedRTL}.

Consider the simple combinational circuit from \figurename~\ref{fig:locality_circuit}.
Based on this circuit, we draw a \textit{locality graph} shown in \figurename~\ref{fig:locality_graph} whose nodes represent the wires of the circuit and each edge between any two nodes represents connectivity of the corresponding two wires through a combinational logic level. 
In other words, each logic gate of the circuit is replaced by multiple edges (three in this case) in the graph which connect together the nodes corresponding to its inputs and the output.
For any two nodes (i.e. wires) $i$ and $j$ in a locality graph, we define $dist(i, j)$ as the shortest distance between $i$ and $j$.
In other words, $dist(i, j)$ represents the minimum number of basic combinational or sequential logic levels (e.g. logic gates and/or flip flops) between wires $i$ and $j$.
E.g. $dist(E, B) = dist(E, C) = 1$, whereas $dist(E, O) = dist(E, A) = 2$.

\begin{definition} \label{def:locality}
\textbf{Trigger Signal Locality \boldmath{$l({\cal T})$}} of a HT represented by the set of trigger states ${\cal T}$ is defined as: 
$$l({\cal T}) = \underset{Trig\in {\cal T}}{\max} \left( \underset{0 \leq i,j < |Trig|}{\max} dist(Trig[i], Trig[j]) \right)$$
where $Trig[i]$ represents the label of the $i_{th}$ wire in $Trig$.
\end{definition}

A low value of $l({\cal T})$ shows that the trigger signal wires of the HT are in the close vicinity of each other and vice versa.
Having a notion of locality can significantly reduce the computational complexity of logic testing based HT detection tools. 

%****************** Achievable Triples  
\subsection{Achievable Quadruples $(d, t,\alpha, l)$}
A Hardware Trojan can be represented by multiple sets of trigger states ${\cal T}$, each having their own $d$, $t$, $\alpha$, and $l$ values.  
The collection of corresponding quadruples $(d,t,\alpha,l)$ is defined as the achievable region of the Hardware Trojan.
%We denote by $H_{d,t,\alpha,l}$ all  $H_D$ type Trojans which can be represented by a set of trigger states ${\cal T}$ with parameters $d({\cal T})\leq d$, $t({\cal T})\leq t$, $\alpha({\cal T})\leq \alpha$ and $l({\cal T})\leq l$.
%In the remainder of this paper we develop HaTCh which takes parameters $t$, $\alpha$ and $d$ as input in order to detect hardware trojans from $H_{t,\alpha,d}$. 
%E.g., by taking $t=0$ we can detect a simple counter-based HT for small $d$ (as we have seen there exists a trigger state $Trig$ for $t=0$ in a simple counter-based HT; HaTCh for $t=0$ will characterize $Trig$ so that malicious behavior can be detected). 
%However, for our more complex $k$\textit{-XOR-LFSR} trojan, HaTCh for $t=0$ only detects this trojan if $d$ is taken $\geq \log k -2\log\log k$.
% which may make HaTCh's computational complexity prohibitive (see Theorem \ref{th:complexity}).

%\subsubsection{Effective Stealthiness: \boldmath{$\alpha^*$}}

The choice of parameters $d$ and $t$ significantly affects $\alpha$ of the HT. % and consequently the detection capability of HaTCh.
%Although reducing $t$ and/or $d$ reduces the memory requirements of the tool and/or computational complexity respectively, it also increases the chances of not detecting the trojan.
%In other words, this can potentially increase the stealthiness factor $\alpha$ of a $H_{t,\alpha,d}$ trojan to $\alpha^* \ge \alpha$.
%We call the probability $\alpha^*$ `effective stealthiness' of the $H_{t,\alpha,d}$ trojan as seen by \Call{HaTCh}{} algorithm as a result of the provided values of parameters $t$ and $d$.
%\figurename~\ref{fig:alpha_tradeoffs} shows the effects of changing $t$ and $d$ on the minimum possible $\alpha$ in the achievable region of a hardware trojan.
$\alpha$ as a function of $t$ and $d$ is decreasing in both $t$ and $d$.
Reducing $t$ means that explicit malicious behavior may not have had the chance to occur, hence, the probability $\alpha$  that no explicit malicious behavior is seen increases. 
Similarly, reducing $d$ can increase $\alpha$ since as a result of smaller $d$, there may not exist a set of trigger signals ${\cal T}$ that represents the HT and satisfies $d({\cal T})\leq d$.
%On the other hand, a higher $d$ incorporates a larger search space and may reduce $\alpha$ down to zero provided that the trojan does not get triggered and manifest implicit malicious behavior during the learning phase.
Increasing $t$ or $d$ only decreases $\alpha$ down to a certain level; the remaining component of $\alpha$ represents the inherent implicit malicious behavior of the HT.


% ==========================================================================
%\subsection{A Counter-Based $H_D$ Trojan}
%
%The HT shown in \figurename~\ref{fig:h2_lfsr_fig} can leak $Secret$ via $Out$ port instead of $Data$ upon the trigger condition $W1\neq W2$.
%The trigger condition is generated by a counter, when reached to ($1101$), which is implemented as a 4-bit maximal LFSR in order to have maximum possible time before the HT gets triggered.
%The LFSR is initialized to $(Q3,Q2,Q1,Q0)=(1010)$ and it can be seen in \figurename~\ref{fig:h2_lfsr_table} that if given the parameter $d=1$, HaTCh will whitelist all the wires related to trigger circuitry only after a few clock cycles since all these wires show transitions.
%At $14th$ clock cycle, the value of the LFSR becomes $(1101)$ and $W1 \neq W2$, which activates the Trojan to leak the secret.
%
%\begin{figure}[!t]
%\centering
%\subfloat[Trojan Circuitry]{\includegraphics[width=2.4in]{h2_lfsr_exp_updated}
%\label{fig:h2_lfsr_fig}}
%%\hfill
%\hspace{0.1in}
%\subfloat[Truth Table of the Trojan affected circuit. Trigger: $W1 \neq W2$]{
%\renewcommand{\arraystretch}{1.2}
%\begin{tabular}[b]{|c||c|c|c|c||c|c|c|}
%\hline
%$Cycle$ & $Q3$ & $Q2$ & $Q1$ & $Q0$ & $W1$ & $W2$ & $W3$ \\
%\hline
%0 & 1 & 0 & 1 & 0 & 1 & 1 & 0\\
%1 & 0 & 1 & 0 & 1 & 0 & 0 & 0\\
%2 & 1 & 0 & 1 & 1 & 1 & 1 & 0\\
%3 & 0 & 1 & 1 & 1 & 1 & 1 & 0\\
%4 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
%5 & 1 & 1 & 1 & 0 & 1 & 1 & 0\\
%6 & 1 & 1 & 0 & 0 & 0 & 0 & 0\\
%7 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\
%8 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\
%9 & 0 & 0 & 1 & 0 & 1 & 1 & 0\\
%10 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\
%11 & 1 & 0 & 0 & 1 & 0 & 0 & 0\\
%12 & 0 & 0 & 1 & 1 & 1 & 1 & 0\\
%13 & 0 & 1 & 1 & 0 & 1 & 1 & 0\\
%\bfseries 14 & \bfseries 1 & \bfseries 1 & \bfseries 0 & \bfseries 1 & \bfseries 0 & \bfseries 1 &\bfseries 1 \\
%\hline
%\end{tabular}
%\label{fig:h2_lfsr_table}
%}
%\caption{A Counter-Based $H_{0,2}$ Trojan to enable the secret leakage}
%\label{fig:h2_lfsr_ex}
%\end{figure}
%
%%\vspace{0.2cm}
%%\subsection{Detection by HaTCh with $d=2$}
%As it is clear from \figurename~\ref{fig:h2_lfsr_table} that, given the parameter $d=1$, this Trojan cannot by detected by HaTCh since all the wires show transitions and get whitelisted after $4th$ clock cycle.
%Therefore we run HaTCh with a parameter $d=2$ in order to show that HaTCh is still able to detect this Trojan.
%With $d=2$, HaTCh exhaustively monitors all possible 2-wire combinations of all the wires in the design.
%It starts with a blacklist of all possible 2-wire combinations (e.g. $\{00,01,10,11\}$) of all the wires in the design and those combinations which are seen during the simulation are removed from the blacklist provided that the output $Out$ matches the expected output for every input.
%
%If the learning phase is run for $13$ clock cycles, then after the optimizations of HaTCh, we only see one combination of $W1$ and $W3$ in the final blacklist i.e. $( W1,W3)=(0,1)$ which only occurs upon the trigger condition. 
%All other redundant combinations are optimized away from the blacklist because the logical constraints of the design never allow these combinations to occur in the future, e.g. $(W1,W2)=(1,0)$ is never possible (unless a stuck at $0$ fault for $W2$).
%Hence HaTCh is able to detect this Trojan.
%Notice that if the learning phase is run for fewer clock cycles, then HaTCh will produce a larger blacklist with more blacklisted combinations.

% ======================================================================

\section{Examples of $H_D$ Trojans}
In this section, we present some examples of new HTs from the class $H_D$.
These HTs demonstrate how the properties of $H_D$ Trojans defined in the previous section play a significant role in determining the stealthiness of these HTs.

\subsection{A Counter-Based $H_D$ Trojan}\label{htd-h2}
\begin{figure}[!t]
\centering
\subfloat[A counter based $H_D$ Trojan. Trigger Condition: $LFSR = 1101$; Trigger Signal: $(W1, W2)$; Payload: Leak $Secret$]{\includegraphics[width=2.4in]{h2_lfsr_exp_updated}
\label{fig:h2_lfsr_fig}}
\hfill
\subfloat[Truth Table of the Trojan affected circuit. Trigger Condition: $LFSR = 1101$]{
\renewcommand{\arraystretch}{1.1}
\begin{tabular}[b]{|c||c|c|c|c||c|c|c|}
\hline
$Cycle$ & $Q3$ & $Q2$ & $Q1$ & $Q0$ & $W1$ & $W2$ & $W3$ \\
\hline
0 & 1 & 0 & 1 & 0 & 1 & 1 & 0\\
1 & 0 & 1 & 0 & 1 & 0 & 0 & 0\\
2 & 1 & 0 & 1 & 1 & 1 & 1 & 0\\
3 & 0 & 1 & 1 & 1 & 1 & 1 & 0\\
4 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
5 & 1 & 1 & 1 & 0 & 1 & 1 & 0\\
6 & 1 & 1 & 0 & 0 & 0 & 0 & 0\\
7 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\
8 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\
9 & 0 & 0 & 1 & 0 & 1 & 1 & 0\\
10 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\
11 & 1 & 0 & 0 & 1 & 0 & 0 & 0\\
12 & 0 & 0 & 1 & 1 & 1 & 1 & 0\\
13 & 0 & 1 & 1 & 0 & 1 & 1 & 0\\
\bfseries 14 & \bfseries 1 & \bfseries 1 & \bfseries 0 & \bfseries 1 & \bfseries 0 & \bfseries 1 &\bfseries 1 \\
\hline
\end{tabular}
\label{fig:h2_lfsr_table}
}
\caption{A Counter-Based $H_D$ Trojan having Trigger Signal Dimension $d=2$.}
\label{fig:h2_lfsr_ex}
\end{figure}

The example Trojan shown in \figurename~\ref{fig:h2_lfsr_fig} can leak $Secret$ via $Out$ port instead of $Data$ once it is activated.
The trigger condition of this Trojan is generated by a counter, when reached to ($1101$), which is implemented as a 4-bit maximal LFSR in order to have maximum possible time before the Trojan gets triggered.
The LFSR is initialized to $(Q3,Q2,Q1,Q0)=(1010)$.
At $14th$ clock cycle, the trigger condition (i.e. $LFSR = 1101$) occurs, the HT gets triggered and produces $W1 \ne W2$ on the trigger signal ($W1, W2$).
This results in the activation of payload circuitry (the group of three MUXes) which leaks the secret.


It can be seen in \figurename~\ref{fig:h2_lfsr_table} that all individual wires related to the HT circuitry are continuously showing transitions \textit{without} activating the HT during several clock cycles before reaching to the trigger condition (i.e. cycle $14$).
Therefore, clearly those existing logic testing based HT detection techniques which only look for simplistic one-dimensional HT (i.e. $d=1$) trigger signals do not see any `suspicious' wire which is stuck at $0$ or $1$, and hence this HT is not detected unless it gets activated in a long testing phase. 
This shows that this HT has a trigger signal dimension $d=2$ since two wires $W1$ and $W2$ together constitute the trigger signal.
Since counter based HTs can have large counters, it may not always be feasible to activate them during testing.
Consequently, in order to efficiently detect such HTs, the knowledge of such design parameters must be incorporated while designing the HT countermeasures.




\subsection{An Advanced $H_D$ Trojan: $k$-\textit{XOR-LFSR}}
\figurename~\ref{fig-htd} depicts $k$-\textit{XOR-LFSR}, a counter based Trojan with the counter implemented as an LFSR 
%(with a primitive feedback polynomial) 
of size $k$. The Trojan is merged with the circuitry of an IP core which outputs the XOR of $k$ inputs $A_j$.

Let ${\bf r}^i\in \{0,1\}^k$  denote the LFSR register content at clock cycle $i$ represented as a binary vector of length $k$. 
Suppose that $u$ is the maximum index for which the linear space $L$ generated by vectors ${\bf r}^0, \ldots, {\bf r}^{u-1}$ (modulo 2) has dimension $k-1$. 
Since  $dim(L)=k-1<k=dim(\{0,1\}^k)$, there exists a vector ${\bf v}\in \{0,1\}^k$ such that, (1) the inner products $\langle {\bf v},{\bf r}^i\rangle=0$ (modulo 2) for all $0\leq i\leq u-1$, and (2) $\langle {\bf v},{\bf r}^u\rangle=1$ (modulo 2). 
{\em Only} the register cells corresponding to ${\bf v}_j=1$ are being XORed with inputs $A_j$. 
%The expected Hamming weight of $v$ is $k/2$, which is the number of XORs of register cells with the $A_j$ as depicted in \figurename~\ref{fig-htd}. 

Since the $A_j$ are all XORed together in the specified  logical functionality to produce the sum $\sum_j A_j$, the Trojan changes this sum to
$$\sum_j A_j \oplus \sum_{j: {\bf v}_j=1} {\bf r}^i_j = \sum_j A_j \oplus \langle {\bf v},{\bf r}^i\rangle.$$
I.e., the sum remains unchanged until the $u$-th clock cycle when it is maliciously inverted.

\begin{figure}[!t]
\centering
\includegraphics[width=2.6in]{general_ht}
\caption{$k$-\textit{XOR-LFSR}: A general $H_D$ Trojan.}
\label{fig-htd}
\end{figure}


The trojan uses an LFSR to generate register values ${\bf r}^i\in \{0,1\}^k$ for each clock cycle $i$ and we assume in our analysis  that all vectors ${\bf r}^i$ behave like random vectors from a uniform distribution. 
Then, it is unlikely that $u$ is more than a small constant larger than $k$ (since every new vector ${\bf r}^i$ has at least probability $1/2$ to increase the dimension by one). 
Therefore, $u\approx k$, hence, the register size of the trojan is comparable to the number of clock cycles before the trojan is triggered to deliver its malicious payload. 
This makes the trojan somewhat contrived (since it can possibly be detected by its suspiciously large area overhead). 

Since inputs $A_j$ can take on any values, any trigger signal $Trig$ must represent a subset of the LFSR register content. Suppose $t(\{Trig\})=j$. Then $Trig$ must represent a subset of ${\bf r}^{u-j}$.
We will proceed with showing a lower bound on $d(\{Trig\})$.
% for 
%the $k$-\textit{XOR-LFSR} trojan. 
%\todo[inline]{We have not defined $L_t(User)$ or $L_0$ yet. Following argument needs to be adapted accordingly.}
%(2) %By our definition of $L_0$, all vectors $r^i$, $0\leq i\leq u-1$, are part of states in $L_0$. 
Consider a projection $P$ to a subset of $d$ register cells; by ${\bf r}|P$ we denote the projection of ${\bf r}$ under $P$, and we call $P$ $d$-dimensional. If ${\bf r}^{u-j}|P \in \{{\bf r}^i|P:0\leq i<u-j\}$, then the wire combination of the  $d$ wires corresponding to ${\bf r}^{u-j}|P$ {\em cannot} represent $Trig$ (otherwise $t(\{Trig\})>j$): if this is the case for all $d$ dimensional $P$, then $Trig$ cannot represent a subset of ${\bf r}^{u-j}$. The probability that  ${\bf r}^{u-j}|P \in \{{\bf r}^i|P:0\leq i<u-j\}$ is at least equal to the probability that $\{{\bf r}^i|P : 0\leq i<u-j\} =\{0,1\}^d$, which is (by the union bound) 
$$\geq 1- \sum_{w\in \{0,1\}^d} Prob(\{{\bf r}^i|P : 0\leq i<u-j\} \subseteq \{0,1\}^d\setminus \{w\})$$
\vspace{-6pt}
$$= 1-\sum_{w\in \{0,1\}^d} (1-1/2^d)^{u-j} \approx 1-2^d e^{-(u-j)/2^d}$$
%\begin{eqnarray*}
%& \geq & 1- \sum_{w\in \{0,1\}^d} Prob(\{{\bf r}^i|P : 0\leq i<u-j\} \subseteq \{0,1\}^d\setminus \{w\}) \\
%& = & 1-\sum_{w\in \{0,1\}^d} (1-1/2^d)^{u-j} \approx 1-2^d e^{-(u-j)/2^d} 
%\end{eqnarray*}
Since there are $\binom{k}{d}\leq k^d/d!$ projections, $Trig$ cannot represent a subset of ${\bf r}^{u-j}$ with probability 
%(taken over all random ${\bf r}^i$)
\begin{equation} \geq (1-2^de^{-(u-j)/2^d})^{k^d/d!} \label{eqLB} \end{equation}
For $d \leq \log (u-j) - \log (\log (u-j) \log k +\log \log k)$,  this lower bound is about $\geq 1/e$.
Since $u\approx k$ and after neglecting the term $\log \log k$, this shows an approximate lower bound on $d(\{Trig\})$, i.e.,
$$\geq \log (k-t(\{Trig\})) - \log (\log (k-t(\{Trig\})) \log k) $$

This characterizes the stealthiness of the $k$-\textit{XOR-LFSR}.
%We prove (cf. section \ref{app-htd}) that $k$-\textit{XOR-LFSR} has
%$$ d(\{Trig\}) \geq \log \big(k-t(\{Trig\})\big) - \log \big(\log (k-t(\{Trig\})) \log k \big) $$
%for any trigger signal $Trig$.
In other words, the stealthiness of $k$-\textit{XOR-LFSR} can be increased with $k$ within the acceptable area overhead limits.
\figurename~\ref{fig:d_bound_XORLFSR} shows the lower bounds on $d$ for this HT for fixed values of $k$ and $t$; if $t(\{Trig\}))=0$, then $d(\{Trig\}) \geq \log k -2\log\log k$.
The HT can be designed for any point in the region above the lower bound.
For the HT shown in \figurename~\ref{fig-htd}, clearly %$t(\{Trig\}))=0$ and 
$\alpha(Trig)=0$ since it \textit{always} produces incorrect output immediately once the HT gets triggered.

\begin{figure}[!t]
\centering
\subfloat[$k=256$]{\includegraphics[width=1.7in]{d_bound_t}
\label{fig:d_bound_t}}
\hfil
\subfloat[$t=0$]{\includegraphics[width=1.7in]{d_bound_k}
\label{fig:d_bound_k}}
\caption{Lower bounds on $d$ for $k$-\textit{XOR-LFSR}.}
\label{fig:d_bound_XORLFSR}
\end{figure}







%\begin{algorithm}[!t]
%\caption{Design a k-XOR-LFSR HT} \label{design_algo}
%\begin{algorithmic}[1]
%\Procedure{k-XOR-LFSR}{$d$}
%	\State $k = 2^d$
%	\ForAll{ $1 \leq i \leq 2^k-1$ }
%		\ForAll { $1 \leq v \leq 2^k-1$ }
%			\If {$HW(v) == d$}
%				\State $r = i, cnt = 0$
%				\State $p = parity (<v,r>)$
%				\While {$p == 0$}
%					\State $cnt$ ++ 
%					\State $r \gets \Call{MXLFSR}{k,r}$
%					\State $p = parity (<v,r>)$
%				\EndWhile
%				\If {$cnt == k - 1$}
%					\State return $i,v$
%				\EndIf
%			\EndIf
%		\EndFor
%	\EndFor
%	\State return $\bot$
%\EndProcedure
%\end{algorithmic}
%\end{algorithm} 


%\vspace{3pt}
%\subsection{Achievable Triples $(t,\alpha,d)$}
%A hardware Trojan can be represented by multiple sets of trigger states ${\cal T}$, each having their own $t$, $\alpha$, and $d$ values.  The collection of corresponding triples $(t,\alpha,d)$ is defined as the achievable region of the hardware Trojan.
%We denote by $H_{t,\alpha,d}$ all  $H_D$ type Trojans which can be represented by a set of trigger states ${\cal T}$ with parameters $t({\cal T})\leq t$, $\alpha({\cal T})\leq \alpha$ and $d({\cal T})\leq d$.
%
%In the remainder of this paper we develop HaTCh which takes parameters $t$, $\alpha$ and $d$ as input in order to detect hardware Trojans from $H_{t,\alpha,d}$. 
%E.g., by taking $t=0$ we can detect a simple counter-based hardware Trojan for small $d$ (as we have seen there exists a trigger state $Trig$ for $t=0$ in a simple counter-based hardware Trojan; HaTCh for $t=0$ will characterize $Trig$ so that malicious behavior can be detected). 
%However, for our more complex $k$\textit{-XOR-LFSR} Trojan, HaTCh for $t=0$ only detects this Trojan if $d$ is taken $\geq \log k -2\log\log k$.
%% which may make HaTCh's computational complexity prohibitive (see Theorem \ref{th:complexity}).
%
%%\subsubsection{Effective Stealthiness: \boldmath{$\alpha^*$}}
%
%The choice of parameters $t$ and $d$ significantly affects $\alpha$ of the HT. % and consequently the detection capability of HaTCh.
%%Although reducing $t$ and/or $d$ reduces the memory requirements of the tool and/or computational complexity respectively, it also increases the chances of not detecting the Trojan.
%%In other words, this can potentially increase the stealthiness factor $\alpha$ of a $H_{t,\alpha,d}$ Trojan to $\alpha^* \ge \alpha$.
%%We call the probability $\alpha^*$ `effective stealthiness' of the $H_{t,\alpha,d}$ Trojan as seen by \Call{HaTCh}{} algorithm as a result of the provided values of parameters $t$ and $d$.
%%\figurename~\ref{fig:alpha_tradeoffs} shows the effects of changing $t$ and $d$ on the minimum possible $\alpha$ in the achievable region of a hardware Trojan.
%$\alpha$ as a function of $t$ and $d$ is decreasing in both $t$ and $d$.
%Reducing $t$ means that explicit malicious behavior may not have had the chance to occur, hence, the probability $\alpha$  that no explicit malicious behavior is seen increases. 
%Similarly, reducing $d$ can increase $\alpha$ since as a result of smaller $d$, there may not exist a set of trigger signals ${\cal T}$ that represents the HT and satisfies $d({\cal T})\leq d$.
%%On the other hand, a higher $d$ incorporates a larger search space and may reduce $\alpha$ down to zero provided that the Trojan does not get triggered and manifest implicit malicious behavior during the learning phase.
%Increasing $t$ or $d$ only decreases $\alpha$ down to a certain level; the remaining component of $\alpha$ represents the inherent implicit malicious behavior of the HT.



%$u\approx k$, this lower bound is about $\geq 1/e$ for $k^d/d!\leq 2^{-d}e^{k/2^d}$, e.g, $d\approx \log k - 2\log\log k$. 
%This shows that $k$-\textit{XOR-LFSR} is $\not\in H_{0, \alpha, \approx \log k - 2\log \log k}$ but is in $\in H_{0, \alpha, d}$ for some larger $d$.
%The \textit{k-XOR-LFSR} Trojan has $d \approx \log k - 2\log \log k$.
%Notice that the dimension $d$ of this Trojan, according to our definitional framework, is independent of the inputs $A_j$.
%Therefore in this sense, the $k$-\textit{XOR-LFSR} Trojan is universally applicable to cores that implement an XOR over $k$ inputs.


%We define $H_t$ as the set of \textit{XX-St-D} Trojans that meet the upper bound $t$. 
%I.e., informally, a core with a hardware Trojan in $H_t$ has the property that if an input sequence manifests malicious behavior, then there must have been a trigger state that
%\begin{enumerate}
%\item Cannot be seen in normal behavior 
%\item Causes the core to manifest malicious behavior after at most $t$ state transitions regardless of any user interactions.
%\end{enumerate}


%\subsubsection{\textit{`l'}: Trigger Signal Locality}
%We first introduce the idea of \textit{locality} in gate level circuits.
%We define locality $l$ between two wires as the minimum distance between them in the gate level netlist in terms of basic combinational or sequential logic levels (e.g. logic gates and flipflops).
%A low value of $l$ shows that the corresponding wires are in the close vicinity of each other and vice versa.
%
%Consider the simple combinational circuit from \figurename~\ref{fig:locality_circuit}.
%Based on this circuit, we draw a \textit{locality graph} shown in \figurename~\ref{fig:locality_graph} whose nodes represent the wires of the circuit and each edge between any two nodes represents connectivity of the corresponding two wires through a combinational logic level. 
%In other words, each logic gate of the circuit is replaced by multiple edges (three in this case) in the graph which connect together the nodes corresponding to its inputs and the output.
%One can easily find the locality of any two wires in the circuit through its locality graph, e.g. $E$ has locality $l=1$ with $B$, $C$, $D$ and $F$ whereas $O$ has locality $l=1$ with $A$ and $F$.
%On the other hand, $E$ has $l=2$ with $A$ and $O$.
%
%For Trojans with multi-bit trigger signals ($d>1$), locality plays an important role in stealthiness of the Trojan.
%The wires of a multi-bit trigger signal which have a high value of $l$ are spread out in the circuit and make it hard to detect such Trojans for the techniques which focus only on regional or local set of wires.

%\begin{figure}[!t]
%\centering
%\subfloat[A simple combinational circuit]{\includegraphics[width=1.2in]{locality_circuit}
%\label{fig:locality_circuit}}
%\hfil
%\subfloat[Locality Graph of the circuit]{\includegraphics[width=1.8in]{locality_graph}
%\label{fig:locality_graph}}
%\caption{Example of Locality Graph: \figurename~\ref{fig:locality_graph} shows the locality graph of the circuit from \figurename~\ref{fig:locality_circuit}. The wires of the circuit are replaced by nodes and the logic gates are replaced by edges to form the locality graph.}
%\label{fig:locality_graph_example}
%\end{figure}



%We will introduce the term ``Effective Stealthiness'' 

%We analyze the probability $\alpha$ in detail in section \ref{sec:hatch_framework}.

%\subsubsection{Hardware Trojan Class $H_{t,\alpha,d}$} \label{sec:Trojan_class}
%%\vspace{0.3cm}
%With these characteristics of hardware Trojans and the intuitions behind the parameters $t$, $\alpha$ and $d$ in mind, now we formally define the Trojans hierarchy $H_{t,\alpha,d}$. 
%
%%\subsubsection{Class $H_{t,\alpha}$}
%Let ${\cal T}$ be a set of trigger states that have the property that  $M^{Core}$ manifests malicious behavior if and only if it has passed through a state in ${\cal T}$.
%Clearly, since ${\cal T}$ is finite, there must be some upper bound $t$ on the number of cycles within which malicious behavior manifests after $M^{Core}$ passes through a state in ${\cal T}$.
%We (informally) define $H_{t,\alpha}$ as the set of \textit{St-D} Trojans that meet the upper bound $t$.
%%A formal definition of $H_t$ is as follows: 
%
%%\begin{definition}%[$H_t$]
%%$Core \in H_t$ if and only if the following conditions hold:
%%\begin{enumerate}[$\mathcal{C}$1)]
%%\item \label{def:ht_item1} There exists a $User$ such that \Call{Simulate}{$Core, User$} outputs ``Trojan-Detected''. I.e., $Core$ is indeed capable of malicious behavior in the form of a violation of the functional spec. 
%%\item \label{def:ht_item2} For all $User$ with the property that \Call{Simulate}{$Core, User$} returns (``Trojan-Detected'', $States$), there exists a state $S=States[j]$ for some $1 \leq j \leq |States|$ such that for all $j'$ and $User'$
%%%$$
%%%\underset{User',J',j'}{\forall}
%%%$$
%%\begin{equation}
%%%\left\{
%%\begin{array}{l}
%%
%%\left[
%%\begin{array}{l}
%%(\mbox{``OK''},States') \gets \Call{Simulate}{Core, User'}\\
%%S = States'[j']
%%\end{array}
%%\right] 
%%\\
%%\Longrightarrow  \\
%%%\underset{User',J',j'}{\forall}
%%\begin{aligned}|States'| &< j'+t\end{aligned}
%%\end{array} \label{eqdef}
%%%\right\}
%%\end{equation}
%%Here, $S$ represents a trigger state after which, independent of any $User'$, either the IP core manifests malicious behavior or the IP core aborts/terminates  in $<t$ clock cycles without eliciting malicious behavior.
%%\end{enumerate}
%%\end{definition}
%
%%\todo[inline]{Maybe we can move the definition of $L_{t}$ up before definition 1 to simplify the ideas.}
% 
%For a formal definition of $H_{t,\alpha}$, we first define the concept of $t$-legitimate states.
%
%\begin{definition}
%	Let $(w,States) \gets \Call{Simulate}{Core, User}$. 
%	Assuming $Core$ is fixed, we define $W(User) =w$ and the set of $t$-legitimate states of $User$ as:
%	$$L_t(User) = \{ States[1], \ldots, States[|States|-t] \}$$
%	(Since \Call{Simulate}{} is deterministic, $L_t(User)$ and $W(User)$ are well-defined.)
%	%We define
%	%$$ L_t = \bigcup_{W(User)=\mbox{``OK''}} L_t(User)$$
%\end{definition}
%
%%\begin{definition} We define the set of $t$-legitimate states of $Core$ as
%%% $$L_t^{Core} = \left\{ S :\begin{array}{l}  \exists_{User, J} \mbox{ such that}  \\  (.,States) \gets \Call{Simulate}{Core, User, J} 
%%%\\ \mbox{where } S=States[j]  \\ \mbox{for some } 1\leq j\leq |States|-t  \end{array} \right\}.$$
%%\begin{equation*}
%%L_t^{Core} =
%%\left \{ S:
%%\begin{aligned}
%%&\underset{User,J}{\exists} \ \ \underset{1\leq j< |States|-t}{\exists} \text{ such that }\\ 
%%&(.,States) \gets \Call{Simulate}{Core,User,J}\\
%%& S = States[j]
%%%&\mbox{where } S = States[j] \text{ for } 1\leq j\leq |States|-t
%%\end{aligned}
%%\right \}
%%\end{equation*}
%%These states can be reached by $M^{Core}$ up to $t$ clock cycles before normal behavior ends or malicious behavior starts manifesting. 
%%\end{definition}
%
%% Let $S_0,S_1, \ldots, S_L$ constitute (the list of) $States$ 
%%as computed by $Emulate[Core]$ in an instantiation of  algorithm \ref{sim_algo}. Then we call each of the states $S_0,S_1, \ldots, S_{L-t}$ {\em $t$-legitimate} for $Core$ if the algorithm outputs ``OK'' (they are at least $t$ clock cycles away from a possible malicious manifestation), and we call each of the states $S_0,S_1, \ldots, S_{L-t-1}$ {\em $t$-legitimate} if the algorithm outputs ``Trojan-Detected'' (these are also at least $t$ clock cycles separated from a possible malicious manifestation).
%
%
%%Let $L_t$ be the set of all $t$-legitimate states. These states can be reached by $M^{Core}$ during normal behavior up to $t$ clock cycles before normal behavior ends or malicious behavior starts manifesting. 
%If a hardware Trojan has the property that it always manifests malicious behavior within $t$ clock cycles after ``it gets triggered'', then we know that the states in $L_t(User)$  do not show the ``trigger signal''. 
%This means that we can use the states in $L_t(User)$ to \textit{whitelist} certain wires (or combinations of wires) from the IP core.
%Now we formalize the definition of $H_{t,\alpha}$:
%
%\begin{definition}
%$Core \in H_{t,\alpha}$ if and only if
%\begin{enumerate}[$\mathcal{C}$1)]
%\item There exists a $User$ and a state $S$ in the set of all reachable states of $M^{Core}$ such that $S \in {\cal T}$. I.e., $Core$ is indeed capable of manifesting malicious behavior.
%\item For all $User$, $\Call{Simulate}{Core, User}$ outputs $W(User)$ such that:
%	\begin{equation*}
%	Prob \left( W(User) = \mbox{``OK''} \; | \; L_t(User) \cap {\cal T} \ne \emptyset \right) = \alpha 
%	\label{eq:alphaDefinition} 
%	\end{equation*}
%\end{enumerate}
%\end{definition}
%
%
%%\begin{definition}
%%$Core \in H_t$ if and only if
%%\begin{enumerate}[$\mathcal{C}$1)]
%%\item \label{lemma:ht_item1} There exists a $User$ such that \Call{Simulate}{$Core, User$} outputs ``Trojan-Detected''. I.e., $Core$ is indeed capable of malicious behavior in the form of a violation of the functional spec.
%%\item \label{lemma:ht_item2} There exists a set ${\cal T}$ of states such that for all $User$:
%%	\begin{eqnarray}
%%	L_0(User)\cap {\cal T} = \emptyset &\Rightarrow& W(User) = \mbox{``OK''} \label{eq:prob0} \\
%%	W(User) = \mbox{``OK''}  &\Rightarrow&  L_t(User)\cap {\cal T} = \emptyset \label{eq:prob1} 
%%	\end{eqnarray}
%%\end{enumerate}
%%\end{definition}
%
%%\begin{proof}
%%$\Rightarrow$: Suppose ``For all $User$ with $W(User)\neq \mbox{``OK''}$ there exists a state $S\in L_0(User)$ such that, for all $User'$, if $W(User')=\mbox{``OK''}$ and $S\in L_0(User')$, then $S\not\in L_t(User')$.'' 
%%Define set ${\cal T}$ as the set of states $S$ for which there exists a $User$ with  $W(User)\neq \mbox{``OK''}$, $S\in L_0(User)$, and the property that, for all $User'$, if $W(User')=\mbox{``OK''}$ and $S\in L_0(User')$, then $S\not\in L_t(User')$. 
%%Now we will prove ($\mathcal{C}$\ref{lemma:ht_item2})  for this particular set ${\cal T}$: 
%%
%%First, let $L_0(User)\cap {\cal T} = \emptyset$. Assume $W(User)\neq \mbox{``OK''}$ then % by definition of $L_t$, 
%%there exists a state $S\in L_0(User)$ such that, for all $User'$, if $W(User')=\mbox{``OK''}$ and $S\in L_0(User')$, then $S\not\in L_t(User')$. 
%%By ${\cal T}$'s definition $S\in {\cal T}$. 
%%This contradicts $L_0(User)\cap {\cal T} = \emptyset$, since $S$ is also in $L_0(User)$. 
%%This means the assumption $W(User)\neq \mbox{``OK''}$ is false.
%%
%%Second, let  $W(User') = \mbox{``OK''}$. 
%%Let $S\in L_t(User')\cap {\cal T}\subseteq L_0(User')\cap {\cal T}$. 
%%Since $S\in {\cal T}$, if $W(User')=\mbox{``OK''}$ and $S\in L_0(User')$, then $S\not\in L_t(User')$ (by definition of ${\cal T}$). 
%%Hence, $S\not\in L_t(User')$, a contradiction. 
%%This shows that $L_t(User')\cap {\cal T}=\emptyset$. 
%%
%%%Second, let $L_0(User')\cap {\cal T} \neq \emptyset$ and  $W(User') = \mbox{``OK''}$. Let $S\in L_0(User')\cap {\cal T}$. Since $S\in {\cal T}$, if $W(User')=\mbox{``OK''}$ and $S\in L_0(User')$, then $S\not\in L_t(User')$ (by ${\cal T}'s definition). Hence, $S\not\in L_t(User')$. This shows that 
%%%$L_t(User')\cap L_0(User')\cap {\cal T}=\emptyset$. Notice that $L_t(User')\subseteq L_0(User')$ and $L_t(User')\cap L_0(User')=L_t(User')$.
%%
%%$\Leftarrow$: Now suppose  ($\mathcal{C}$\ref{lemma:ht_item2}) holds.  
%%We need to prove the statement ``For all $User$ with $W(User)\neq \mbox{``OK''}$ there exists a state $S\in L_0(User)$ such that, for all $User'$, if $W(User')=\mbox{``OK''}$ and $S\in L_0(User')$, then $S\not\in L_t(User')$.'' 
%%Let $W(User)\neq \mbox{``OK''}$, then (\ref{eq:prob0}) implies that there exists a state $S\in L_0(User)\cap {\cal T} $. 
%%Suppose that $W(User')=\mbox{``OK''}$ and $S\in L_0(User')$. 
%%Then 
%%%$S\in L_0(User')\cap {\cal T}$ and 
%%(\ref{eq:prob1}) implies $L_t(User')\cap {\cal T}=\emptyset$, in particular, $S\not\in L_t(User')$.
%%\end{proof}
%
%%Notice that (\ref{eq:prob0}) and (\ref{eq:prob1}) are equivalent to
%%\begin{eqnarray}
%%&& W(User) \neq  \mbox{``OK''}\Rightarrow  L_0(User)\cap {\cal T} \neq \emptyset  \label{prob2} \\
%%&& L_t \cap T = \emptyset. \label{prob3}
%%\end{eqnarray}
%%Together with the previous lemma this proves:
%%
%%\begin{lemma}  
%%$Core \in H_t$ if and only if 
%%\begin{enumerate}[$\mathcal{C}$1*)]
%%\item \label{lemmaDirect:ht_item1} ($\mathcal{C}$\ref{lemma:ht_item1}) holds.
%%\item \label{lemmaDirect:ht_item2} For all $User$ with $W(User)\neq \mbox{``OK''}$, there exists a state $S\in L_0(User)$ such that $S\not\in L_t$.
%%\end{enumerate}
%%\end{lemma}
%
%%\vspace{-0.3cm}
%%For completeness we also give a more direct proof:
%
%%\begin{proof}
%%Suppose ($\mathcal{C}$\ref{def:ht_item2}) holds.
%%Let $W(User)\neq \mbox{``OK''}$. 
%%From ($\mathcal{C}$\ref{def:ht_item2}) we infer that there exists a state $S\in L_0(User)$ such that (\ref{eqdef}) holds for all $User'$ and $j'$.
%%If $S\in L_t$, then by its definition there exists a $User'$ with $W(User')=\mbox{``OK''}$ such that \Call{Simulate}{$Core, User'$} outputs $States'$ with $S=States'[j']$ for some $1\leq j'\leq |States'|-t$.
%%From ($\mathcal{C}$\ref{def:ht_item2}) we infer that $|States'|< j'+t$, a contradiction, hence, $S\not\in L_t$ implying ($\mathcal{C}$\ref{lemma:ht_item2}*).
%%
%%Suppose ($\mathcal{C}$\ref{lemma:ht_item2}*) holds.
%%Suppose the negation of ($\mathcal{C}$\ref{def:ht_item2}), i.e., there exists a $User$ with $W(User) \neq \mbox{``OK''}$ such that for all $S \in L_0(User)$, there exists a $User'$ and $j'$ such that $(\mbox{``OK''}, States')\gets\Call{Simulate}{Core, User'}$ with $S=States'[j']$ and $1\leq j'\leq |States'|-t$.
%%I.e. $S \in L_t(User') \subseteq L_t$.
%%This proves there exists a $User$ with $W(User) \neq \mbox{``OK''}$ such that $S \in L_t$ for all $S \in L_0(User)$ which contradicts ($\mathcal{C}$\ref{lemma:ht_item2}*).
%%\end{proof}
%
%%\begin{lemma}  
%%$Core \in H_t$ if and only if %the following conditions hold:
%%\begin{enumerate}[$\mathcal{C}$1*)]
%%\item \label{lemma:ht_item1} ($\mathcal{C}$\ref{def:ht_item1}) holds.
%%\item \label{lemma:ht_item2} For all $User$ with the property that \Call{Simulate}{$Core, User$} outputs (``Trojan-Detected'', $States$), there exists an index $|States|-t\leq j \leq |States|$ such that state $States[j]\not\in L_t$.
%%\end{enumerate}
%%\end{lemma}
%%
%%\begin{proof}
%%Suppose ($\mathcal{C}$\ref{def:ht_item2}) holds. 
%%If $S\in L_t$, then by its definition there exists a $User'$ and number of rounds $J'$ such that \Call{Simulate}{$Core, User', J'$} outputs $States'$ with $S=States'[j']$ for some  $1\leq j'< |States'|-t$. 
%%From ($\mathcal{C}$\ref{def:ht_item2}) we infer that $|States'|\leq j'+t$, a contradiction, hence, $S\not\in L_t$ implying ($\mathcal{C}$\ref{lemma:ht_item2}*).
%%
%%Suppose ($\mathcal{C}$\ref{lemma:ht_item2}*) holds. 
%%Suppose the negation of ($\mathcal{C}$\ref{def:ht_item2}), i.e., there exists a $User'$, $J'$, and $j'$ such that \Call{Simulate}{$Core, User', J'$} outputs $States'$ with $S=States'[j']$ for some $1\leq j'< |States'|-t$.
%%Then $S\in L_t$ contradicting ($\mathcal{C}$\ref{lemma:ht_item2}*).
%%\end{proof}
%
%%\subsubsection{Introducing The Probability $\alpha$}
%%Since $L_t(User)\subseteq L_0(User)$ we  notice that implication (\ref{eq:prob1}) is equivalent to the implication
%%\begin{equation*}
%%\begin{aligned}
%%& [ W(User) = \mbox{``OK''}  \wedge L_0(User)\cap {\cal T}\neq \emptyset ] \\
%%& \Rightarrow L_t(User)\cap {\cal T} = \emptyset
%%\end{aligned}
%%\end{equation*}
%%which in turn is equivalent to
%%\begin{equation*}
%%Prob \left ( L_t(User)\cap {\cal T} \neq \emptyset \left | 
%%	\begin{aligned}
%%	& W(User) = \mbox{``OK''} , \\
%%	& L_0(User)\cap {\cal T}\neq \emptyset
%%	\end{aligned} \right. \right) =0
%%\end{equation*}
%%
%%The latter implies
%%\begin{equation*}
%%\alpha = Prob \left( \left.
%%	\begin{aligned}
%%	& L_t(User)\cap {\cal T} \neq \emptyset, \\
%%	& W(User) = \mbox{``OK''}  
%%	\end{aligned} \right|  
%%L_0(User)\cap {\cal T}\neq \emptyset \right) = 0
%%\end{equation*}
%
%
%%We may relax our definition by allowing $\alpha>0$. 
%We refer to $\alpha$ as the stealthiness factor of the hardware Trojan (cf. section \ref{subsec:aplha}).
%Notice that if a trigger state occurs and no malicious behavior is manifested, then it seems unlikely that a trigger state occurred before $t$ clock cycles prior to termination: if such a trigger state had occurred in the last $t$ cycles window, it seems that it had enough time ($\geq t$ clock cycles) to propagate malicious behavior to the output port. 
%For this reason, we expect $\alpha$ to be close to $0$ for large enough $t$.
%However, we observe that in general $\alpha>0$ since the caused malicious behavior may coincidentally be the same as normal behavior (recall explicit vs. implicit malicious behaviors from section \ref{subsec:imp-exp-behav}).
%
%
%%\subsubsection{Class $H_{t,\alpha,d}$}
%As explained earlier, hardware Trojans may have multi-bit trigger signals that involve, say, $d$ wires.
%Therefore it is useful to define projections:
%
%\begin{definition}
%We define a vector \textbf{z} projected to index set $P$ as 
%$\mathbf{z}|P = (z_{i_1}, z_{i_2}, \dots, z_{i_d})$
%where $P=\{ i_1, i_2, \dots, i_d \}$ and $i_1 < i_2 < \dots < i_d$. 
%We call $d$ the dimension of projection $P$ and we define ${\cal P}_d$ to be the set of all projections of dimension $d$.
%We define a set $Z$ projected to index set $P$ as 
%$Z|P = \{\mathbf{z}|P : \mathbf{z} \in Z\}$
%\end{definition}
%
%Projections allow us to define the subclass $H_{t,\alpha,d}$:
%\begin{definition}
%$H_{t,\alpha,d}$ consists of $Core\in H_{t,\alpha}$ if for all $User$ with $W(User)\neq \mbox{``OK''}$, there exists a state $S\in L_t(User)$ and a projection $P\in {\cal P}_d$ such that $S|P\not\in L_t(User)|P$.
%%I.e., $(P,S|P)\not\in W_{t,d}$ or equivalently $(P,S|P)\in B_{t,d}$. 
%\end{definition}
%
%If $Core \in H_{t,\alpha,d}$, then trigger states $S$ manifest themselves as a unique value of $d$ wires in a way that is never observed during the normal behavior (i.e., a rare trigger condition).
%The notion of dimension $d$ paves the path to design a Trojan detection tool.
%On one hand, it provides a mechanism to detect the trigger states of the hardware Trojan by monitoring only $d$ dimensional projections of state vectors rather than the complete state vectors.
%On the other hand, it directly affects the projections search space for the countermeasure tool.
%%Notice that $H_{t,1}\subseteq H_{t,2}\subseteq \ldots \subseteq H_t$.
%
%%\subsubsection{Whitelist $W_{t,d}$ \& Blacklist $B_{t,d}$}
%%As next steps to design a countermeasure to detect $H_{t,\alpha,d}$ Trojans, we define the whitelist $W_{t,d}$ and its corresponding blacklist $B_{t,d}$ based on the output of $\Call{Simulate}{Core, User}$. 
%%We remind the reader that $S$ represents a state {\em vector}, not a set.
%%
%%\begin{definition}
%%%Whitelist $W_{t,d}$ and blacklist $B_{t,d}$ are defined as:
%%\begin{equation*}
%%\begin{aligned}
%%W_{t,d} &= \{ (P, S|P) \ : \ P\in {\cal P}_d \;,\; S\in L_{t}(User) \} \\ 
%%B_{t,d} &= ({\cal P}_d \times \{0,1\}^d) \setminus W_{t,d}
%%\end{aligned}
%%\end{equation*}
%%\end{definition}
%
%%\vspace{.2cm}
%%We observe that $S\not\in L_t$ is equivalent to
%%$$\exists_d \exists_{P\in {\cal P}_d} \ S|P \not\in L_t|P$$
%%I.e. $S\not\in L_t$ implies $S|P\not\in L_t|P$ for the identity projection which leaves states unchanged; if $S|P\not\in L_t|P$ then $S\not\in L_t$ by the definition of projection $L_t|P$.
%
%
%%At this point, we define the notion of locality $l$ for $H_{t,d}$ Trojans which gives rise to their further subclasses denoted by $H_{t,d,l}$.
%%
%%\begin{definition}
%%$H_{t,d,l}$ consists of $Core\in H_{t,d}$ having a locality graph $G$ with the trigger signal bits $b_1, b_2, \ldots , b_d$ as its nodes along with the other nodes (wires) such that: 
%%$$l = \max \left( \underset{\substack{1 \leq i \leq d \\ 1 \leq j \leq d \\ i < j}}{\forall}\; mindist(b_i,b_j) \right)$$
%%where $mindist(b_i,b_j)$ shows the minimum distance from node $b_i$ to $b_j$ on the locality graph $G$.
%%\end{definition}
%%
%%In other words, $l$ shows the maximum of all $d \choose 2$ shortest distances (in terms of basic combinational or sequential logic levels) for all $d$ wires of the trigger signal.
%%Here $H_{t,d,1}\subseteq H_{t,d,2}\subseteq \ldots \subseteq H_{t,d}$.
%%Since $l$ shows maximum spread of the trigger signal wires in the circuit therefore with the knowledge of $l$, Trojan detection tools, such as HaTCh itself, can become more efficient by only monitoring regions of locality $l$ at a time instead of the whole design.
%%%We will further discuss the significance of locality in section \ref{sec:hatch_framework}.
%
%%Notice that the ${\cal P}_d$, $W_{t,d}$ and $B_{t,d}$ can also be defined for locality $l$ as ${\cal P}_{d,l}$, $W_{t,d,l}$ and $B_{t,d,l}$ respectively.
%%However ${\cal P}_{d,l} \subseteq {\cal P}_d$ because of which by definition $W_{t,d,l} \subseteq W_{t,d}$ and $B_{t,d,l} \subseteq B_{t,d}$.
%%These reduced sizes of sets $W_{t,d,l}$ and $B_{t,d,l}$ lead to a smaller search space for HaTCh resulting in lower complexity and area overhead.
%%On the other hand, these optimizations offer tradeoffs between false positives and false negatives which we discuss in section \ref{sec:hatch_framework}.
%
%%********************************************************************%	
%%\subsection{$H_{0,2}$ Class Trojan Example}
%%In section \ref{sec:background-org}, we have shown an example of a simple $H_{0,2}$ hardware Trojan in \figurename~\ref{fig:simple_ht_exp_2}.
%%In this circuitry, one can only distinguish between the normal behavior and a trigger event with 100\% guarantee by observing the boolean values of 2-wire combinations, hence it has $d=2$. 
%%Specifically $(Sel, A) = (1,1)$ never occurs during the normal operation.
%%As this Trojan exhibits its malicious behavior immediately after the trigger event occurs it has $t=0$.
%%
%%\figurename~\ref{fig:h2_Trojan_ex1} shows another implementation of the same Trojan, having the trigger condition $\{A,B\}=\{1,1\}$, from the previous example.
%%Here, the circuitry from \figurename~\ref{fig:simple_ht_exp_2} is optimized in a way that Trojan circuitry is merged into the normal circuitry.
%%Therefore all the internal wires are part of producing the normal results as well as  is evident from the table in \figurename~\ref{fig:h2_Trojan_ex1_table}.
%%Hence one cannot distinguish the trigger condition by observing individual wires or 1-wire combinations.
%%However, certain 2-wire combinations in this design only occur upon the trigger condition, for example $\{A,B\}=\{1,1\}$, $\{B,A'\}=\{1,0\}$ and $\{B,A'B\}=\{1,0\}$.
%%Since one can only distinguish between the normal behavior and the trigger event of this Trojan by observing 2-wire combinations, and since it shows malicious behavior immediately after the trigger condition,  it is also a $H_{0,2}$ Trojan.
%%
%%For completeness, we mention that DeTrust in their recent paper (section $3.3$ in \cite{detrust}) created a Trojan design  which turns out to be in $H_{1,2}$ according to our hierarchical model.
%%
%%We also show another example of a counter based $H_{0,2}$ Trojan in Appendix \ref{app-htd-h2}.
%%
%%\begin{figure}[!t]
%%\centering
%%\subfloat[$S=A\oplus B$ affected to produce $S=A+A'B$]{\includegraphics[width=2in]{h2_Trojan_ex1}
%%\label{fig:h2_Trojan_ex1_fig}}
%%%\hfill
%%\hspace{1in}
%%\subfloat[Truth Table of the Trojan affected circuit. Trigger: $\{A,B\}=\{1,1\}$]{
%%\renewcommand{\arraystretch}{1.2}
%%\begin{tabular}[b]{|c|c||c|c|c|}
%%\hline
%%$A$ & $B$ & $A'$ & $A'B$ & $S$ \\
%%\hline
%%0 & 0 & 1 & 0 & 0\\
%%0 & 1 & 1 & 1 & 1\\
%%1 & 0 & 0 & 0 & 1\\
%%\bfseries 1 & \bfseries 1 & \bfseries 0 & \bfseries 0 & \bfseries 1\\
%%\hline
%%\end{tabular}
%%\label{fig:h2_Trojan_ex1_table}
%%}
%%\caption{A $H_{0,2}$ Trojan embedded in summation function of a Half Adder: 
%%\figurename~\ref{fig:h2_Trojan_ex1_fig} shows the Trojan from \figurename~\ref{fig:simple_ht_exp_2} implemented in a way that the Trojan circuitry cannot be distinguished from the normal circuitry, i.e. there is no single wire which only toggles under trigger condition. This can be seen in the truth table of \figurename~\ref{fig:h2_Trojan_ex1_table}.}
%%\label{fig:h2_Trojan_ex1}
%%\end{figure}
%
%
%%\subsection{$H_{0,d}$ Class Trojan Example} \label{sec-htd}
%%
%%\begin{figure}[!t]
%%\centering
%%\includegraphics[width=2.0in]{general_ht}
%%\caption{$k$-\textit{XOR-LFSR}: A general $H_{t,d}$ hardware Trojan.}
%%\label{fig-htd}
%%\end{figure}
%%
%%Figure \ref{fig-htd} depicts $k$-\textit{XOR-LFSR}, a counter based Trojan with the counter implemented as an LFSR (with a primitive feedback polynomial) of size $k$. Let $r^i\in \{0,1\}^k$  denote its register content at clock cycle $i$ represented as a binary vector of length $k$. Suppose that $u$ is the maximum index for which the linear space $L$ generated by vectors $r^0, \ldots, r^{u-1}$ (modulo 2) has dimension $k-1$. Since  $dim(L)=k-1<k=dim(\{0,1\}^k)$, there exists a vector $v\in \{0,1\}^k$ such that (1) the inner products $\langle v,r^i\rangle=0$ (modulo 2) for all $0\leq i\leq u-1$ and (2) $\langle v,r^u\rangle=1$ (modulo 2). Only the register cells corresponding to $v_j=1$ are being XORed with inputs $A_j$. The expected Hamming weight of $v$ is $k/2$, which is the number of XORs of register cells with the $A_j$ as depicted in figure \ref{fig-htd}. 
%%
%%Since the $A_j$ are all XORed together in the specified  logical functionality to produce the sum $\sum_j A_j$, the Trojan changes this sum to
%%$$\sum_j A_j \oplus \sum_{j: v_j=1} r^i_j = \sum_j A_j \oplus \langle v,r^i\rangle.$$
%%I.e., the sum remains unchanged until the $u$-th clock cycle when it is maliciously inverted. 
%%Notice that the dimension $d$ of this Trojan, according to our definitional framework, is independent of the inputs $A_j$.
%%Therefore in this sense, the $k$-\textit{XOR-LFSR} Trojan is universally applicable to cores that implement an XOR over $k$ inputs.
%%
%%For the proof of the following lemma, see appendix \ref{app-htd-c}.
%%% (it takes $\approx log k$ cycles to propagate the values $r^u_j$ into the sum). I.e, the Trojan is in $H_{t\approx \log k}$.
%%
%%\begin{lemma} Suppose that all vectors $r^i$ behave like random vectors from a uniform distribution.  Then $k$-\textit{XOR-LFSR} has register size $k$ and triggers after $u\approx k$ clock cycles.
%%Furthermore,  $k$-\textit{XOR-LFSR} is $\not\in H_{0, \approx \log k - 2\log \log k}$ but is in $\in H_{0, d}$ for some larger $d$.
%%\end{lemma}
%
%
%
%%********************************************************************%
%%=================================================================================================






